Defensive Approximation: Securing CNNs using Approximate Computing

In the past few years, an increasing number of machine-learning and deep learning structures, such as Convolutional Neural Networks (CNNs), have been applied to solving a wide range of real-life problems. However, these architectures are vulnerable to adversarial attacks. In this paper, we propose for the first time to use hardware-supported approximate computing to improve the robustness of machine learning classifiers. We show that our approximate computing implementation achieves robustness across a wide range of attack scenarios. Specifically, for black-box and grey-box attack scenarios, we show that successful adversarial attacks against the exact classifier have poor transferability to the approximate implementation. Surprisingly, the robustness advantages also apply to white-box attacks where the attacker has access to the internal implementation of the approximate classifier. We explain some of the possible reasons for this robustness through analysis of the internal operation of the approximate implementation. Furthermore, our approximate computing model maintains the same level in terms of classification accuracy, does not require retraining, and reduces resource utilization and energy consumption of the CNN. We conducted extensive experiments on a set of strong adversarial attacks; We empirically show that the proposed implementation increases the robustness of a LeNet-5 and an Alexnet CNNs by up to 99% and 87%, respectively for strong grey-box adversarial attacks along with up to 67% saving in energy consumption due to the simpler nature of the approximate logic. We also show that a white-box attack requires a remarkably higher noise budget to fool the approximate classifier, causing an average of 4db degradation of the PSNR of the input image relative to the images that succeed in fooling the exact classifier

==> asplos21main-p898-p (Copy)/Background.tex <==
This section first presents an overview of adversarial attacks followed by introducing AC.  

% \subsection{Convolutional neural networks}

% A convolutional neural network (CNN) \cite{Alexnet} is a Deep Learning algorithm that takes an image as input, automatically extracts features, and produces labels (corresponding to the classification task the CNN was trained for) as output. 
% A CNN consists of convolution layers and sub-sampling layers performing the feature extraction, followed by fully connected layers performing the classification. The input image is fed to the CNN and the convolution layer creates feature maps. The feature maps are pooled (down-sampled) to reduce their dimension while conserving the most important information, which is one of the factors that make CNNs more tolerant to distortions. The fully connected layers use the feature matrix to classify the input. %Another important concept of CNNs is the use of activation functions, commonly a rectified linear unit (ReLU). Applying a non-saturating ReLU activation function $ ReLu(x)=\max(0,x)$ removes negative values from an activation map by setting them to zero. This increases the nonlinear properties of the decision function and of the overall network without affecting the receptive fields of the convolution layer.

\subsection{Adversarial Attacks}

Deep learning techniques gained popularity in recent years and are now deployed even in safety-critical tasks, such as recognizing road signs for autonomous vehicles \cite{signs}. Despite their effectiveness and popularity, CNN-powered applications are facing a critical challenge – adversarial attacks. Many studies \cite{vulnerable, fgsm, He, neuroattack} have shown that CNNs are vulnerable to carefully crafted inputs designed to fool them, very small imperceptible perturbations added to the data can completely change the output of the model. In computer vision domain, these adversarial examples are intentionally generated images that look almost exactly the same as the original images, but can mislead the classifier to provide wrong prediction outputs. Other work \cite{noneed} claimed that adversarial examples are not a practical threat to ML in real-life scenarios. However, physical adversarial attacks have recently been shown to be effective against CNN based applications in real-world \cite{phys}.

\noindent 
{\bf Minimizing Injected Noise:} Its essential for the adversary to minimize the added noise to avoid detection.  
%, an adversary, using information learned about the structure of the classifier, tries to craft perturbations added to the input to cause incorrect classification.   In these types of attacks, the adversary desires to minimize this perturbation noise to avoid detection.  
For illustration purposes, consider a CNN used for image classification.  More formally, given an original input image $x$ and a target classification model $ f() ~s.t. ~ f(x) = l $, the problem of generating an adversarial example $x^*$ can be formulated as a constrained optimization \cite{pbform}:

\begin{equation}
\label{eq:adv}
     \begin{array}{rlclcl}
        x^* = \displaystyle \argmin_{x^*}  \mathcal{D}(x,x^*),  
         s.t.  ~ f(x^*) = l^*,  ~ l \neq l^*
\end{array}
\end{equation}


Where $\mathcal{D}$ is the distance metric used to quantify the similarity between two images and the goal of the optimization is to minimize this added noise, typically to avoid detection of the adversarial perturbations. $l$ and $l^*$ are the two labels of $x$ and $x^*$, respectively:  $x^*$ is considered as an adversarial example if and only if the label of the two images are different ($ f(x) \neq  f(x^*) $) and the added noise is bounded ($\mathcal{D}(x,x^*) < \epsilon $ where $\epsilon \geqslant 0 $).

%\subsection{Distance metrics}
\noindent
{\bf Distance Metrics:}
The adversarial examples and the added perturbations should be visually imperceptible by humans. Since it is hard to model humans' perception, researchers proposed three metrics to approximate humans' perception of visual difference, namely $L_0$, $L_2$, and $L_ \infty$ \cite{CW}. These metrics are special cases of the $L_p$ norm: 
\begin{equation}
    \left\|x\right\|_p = \left( \sum^{n}_{i = 1} \left |x_i \right | ^{p} \right)^{\frac{1}{p}}
\end{equation}
These three metrics focus on different aspects of visual significance. $L_0$ counts the number of pixels with different values at corresponding positions in the two images. $L_2$ measures the Euclidean distance between the two images $x$ and $x^*$. $L_ \infty$ measures the maximum difference for all pixels at corresponding positions in the two images.


The consequences of an adversarial attack can be dramatic.  For example, misclassification of a stop sign as a yield sign or a speed limit sign could lead to material and human damages. Another possible situation is when using CNNs in financial transactions and automatic bank check processing -- using handwritten character recognition algorithms to read digits from bank cheques or using neural networks for amount and signature recognition \cite{cheque}. An attacker could easily fool the model to predict wrong bank account numbers or amount of money or even fake a signature. A dangerous situation, especially with such large sums of money at stake.

%Still in the financial sector, companies frequently use graph convolutional networks (GCNs) \cite{kipf} to decide whether their customers are trustworthy or not. If scammers succeed in hiding their personal identity information, and avoid company's detection, this will result in a significant loss to the company. Therefore, the security issues of deep neural networks represents a major concern.


\subsection{Approximate Computing}

The speed of new generations of computing systems, from embedded and mobile devices to servers and computing data centers, has been drastically climbing in the past decades. This development was made possible by the advances in integrated circuits (ICs) design and driven by the increasingly high demand for performance in the majority of modern applications. However, this development is physically reaching the end of Moore’s law, since TSMC and Samsung are releasing 5 $nm$ technology \cite{tsmc_moore}. On the other hand, a wide range of modern applications is inherently fault-tolerant and may not require the highest accuracy. This observation has motivated the development of approximate computing (AC), a computing paradigm that trades power consumption with accuracy. The idea is to implement inexact/AC elements that consume less energy, as far as the overall application tolerates the imprecision level in computation.
This paradigm has been shown promising for inherently fault-tolerant applications such as deep/ML, big data analytics, and signal processing. Several AC techniques have been proposed in the literature and can be classified into three main categories based on the computing stack layer they target: software, architecture, and circuit level~\cite{Survey}. 

In this paper, we consider AC for a \emph{totally new objective}; enhancing CNNs robustness to adversarial attacks, without losing the initial advantages of AC.

==> asplos21main-p898-p (Copy)/Conclusions.tex <==

To the best of our knowledge, this is the first work that proposes the use of hardware-supported approximation as a defense strategy against adversarial attacks for CNNs.  
We propose a CNN implementation based on Ax-FPM, an energy-efficient approximate floating-point multiplier. While AC is used in the literature to reduce the energy and delay of CNNs, we show that AC also enhances their robustness to adversarial attacks. The proposed defense is, on average, $87\%$ more robust against strong grey-box attacks and $87.5\%$ against strong black-box attacks than a conventional CNN for the case of MNIST dataset, with negligible loss in accuracy.  %. In terms of accuracy, our results proved that the accuracy drop of an Ax-FPM based CNN is negligible ($0.16\%$), which makes it even more difficult to recognize based on system-level performance. 
%\ihsen{please double check these numbers}
The approximate CNN achieves a significant reduction in power and delay of $50\%$ and $67\%$, respectively. 

%\ihsen{unable to focus for now, please recheck this, it's no longer the case}
%Our future work, pursues several remaining directions: % First, we will consider a white-box attack where the attacker also knows the internal structure of the network; we expect attack transferability to increase under this condition.  
%First, a study on the decision boundaries/regions of a model (size and shape) and a comprehensive analysis of the neighborhood around the input point will be conducted giving a clearer vision of the way approximation is enhancing the robustness and will help in building stronger models.


%In future work, we plan to further mitigate the impact of the adversarial example; we intend to design and deploy randomly reconfigurable AC elements to enhance the resiliency of the CNN.  We also intend to study the generalization of our observations to more complex CNN architectures.


==> asplos21main-p898-p (Copy)/Discussion.tex <==

This work tackles the problem of robustness to adversarial attacks from a new perspective: approximation in the underlying hardware. DA exploits the inherent fault tolerance of deep learning systems \cite{iccd18} to provide resilience while also obtaining the by-product gains of AC in terms of energy and resources. Our empirical study shows promising results in terms of robustness across a wide range of attack scenarios. We notice that AC-induced perturbations tend to help the classifier generalize and enhances its confidence.  We believe that this observation is possibly due to the specific AC multiplier we used where the introduced noise is input-dependent and non-uniform.
When we observe the effect on the convolution layer, we see higher absolute values when the inputs are similar to the convolution filter. This observation at the feature map propagates through the model and results in enhanced classification confidence, i.e., the difference between the $1^{st}$  and  runner-up classes. 
This aspect of confidence enhancement resembles the smoothing effect observed by some recently proposed randomization techniques~\cite{snP2019_certif}.  

 We believe that our study makes important contributions in demonstrating the general potential of approximate computing in this new dimension.  However, we believe that substantial further research remains which we hope to tackle in our future work:  (1) More work is needed to carefully understand the relationship between the patterns of induced noise and the observed robustness to adversarial attacks to guide the selection of approximation approaches; (2) We would also like to explore whether there is additional protection that results from adapting the approximation function over time; (3) We believe that DA is orthogonal to some of the other AML defenses and, deployed together, they may result in even higher protection against AML; (4) Some AML defenses unintentionally make the model more susceptible to privacy related attacks~\cite{rezaShokry}; we believe that DA does not have a similar effect and would like to study its implication on privacy-preserving in the future; and (5) We would like to explore DA in the context of other learning structures beyond CNNs.
 
 %While we do not claim a full and definitive explanation of this mechanism, we believe that the circuit-level approximate mantissa multiplier has a positive effect on the features highlighting. 

%We think that this work opens a new research direction in tackling the deep learning security problem and encourages researchers to investigate further the use of AC as a potential defense mechanism against adversarial attacks. Besides, we believe that the AC-induced noise can also be useful in a privacy preserving context.%, especially in the ca attacks such as membership inference attacks. 

DA has two important advantages compared to DQ: (1) DA results in input-dependent noise, while DQ results in a deterministic network that can be efficiently reverse engineered and undermined by adaptive white-box attacks; (2) DQ requires retraining/fine-tuning the model to avoid drastic accuracy drop, while DA does not require retraining.

Compared to DA, when proceeding to Bfloat16 quantization, we did not notice any improvement in the model robustness, which could be explained by the fact that Bfloat16 results in uniform low-amplitude noise distribution that is not sufficient to impact CNNs behavior.


While  we considered full precision floating point CNNs, we believe that DA can also apply to  quantized and sparse networks~\cite{quant,survey_121,NIPS2018_sparce} with similar impact on security. Prior work~\cite{D&T} shows that quantized networks tolerate errors, implying that DA can potentially be deployed without degrading accuracy.  %Furthermore, we believe that the robustness enhancement introduced by hardware-supported approximation is orthogonal to some other existing robustness approaches (e.g., input reprocessing and adversarial training) and hence could be used in parallel. However, further investigation needs to be done. 

Our experimental setup is based on simulating a cross-layer implementation from gate-level up to system-level. Therefore, the experiments are  computationally and time demanding, which limited our experiments to the two datasets MNIST and CIFAR-10. This limitation was the same for techniques that require Monte Carlo Simulations such as \cite{snP2019_certif}. 
Our observations held for 5-layer-CNN (LeNet) and 8-layer-CNN (AlexNet). In future work, we are planning to solve the simulation time limitation by a real hardware implementation, which facilitate evaluating DA for larger networks.  %Therefore, we believe that further experiments on deeper networks should confirm our current findings.


%This aspect enhances CNNs robustness to adversarial attacks. The modified approximate decision boundary prevents transferability of adversarial examples generated under black-box and gray-box settings. In a white-box setting, we demonstrated that an adversarial example generated for the approximate model requires higher distance to the clean sample, and consequently higher noise magnitude. In other words, an adversary needs to make his example more detectable by a human eye, which weakens his attack. 
%Moreover, the choice of the data-driven approximate FA sharpens the correlation between the noise and the input data, which makes the approximation behave as a separate channel superimposed to the initial classifier. 
%Future work will consider newer attacks such as C\&W, PDG and HopSkipJump attacks as well as architectures with higher complexity.

%\ihsen{Mention Leaky Relu, stochastic, summarize the advantages in implementation, Differential Privacy (Monte carlo simulation), privacy}

==> asplos21main-p898-p (Copy)/Introduction.tex <==

Convolutional neural networks (CNNs) and other deep learning structures  provide state-of-the-art performance in many application domains, such as computer vision \cite{simonyan2014deep,redmon2016yolo9000}, natural language processing \cite{deng2018deep}, robotics \cite{pierson2017deep}, autonomous driving \cite{al2017deep}, and healthcare \cite{miotto2018deep}. With the rapid progress in CNN's development and deployment, they are increasing concerns about their vulnerability to adversarial attacks: maliciously designed imperceptible perturbations injected within the data that cause CNNs to misclassify.   Adversarial attacks have been demonstrated in real-world scenarios \cite {phy9,phy10,neuroattack}, making this vulnerability a serious threat to safety-critical and other applications that rely on CNNs. %In fact, it is possible to craft adversarial examples that generalize to the real world under different orientations and lighting conditions. 
%bNs). y showing that whe(DNn printed out, an adversarially constructed image will continue to fool neural networks under different lighting and orientations.
%As a result, adversarial attacks have to be taken into account while developing safety and security-critical applications incorporating CNNs. 

%%Since the demonstration of adversarial examples, several attacks and defenses have been proposed.  %, each building on one another. Previous work proposed solutions based on manipulating either the input data, the objective function, or the network structure to mitigate adversarial effects. However, these proposed techniques require substantial changes to the architecture, retraining procedure, or incorporate additional input data processing overhead.  In addition, some proposed defenses have been shown to be vulnerable to alternative attack strategies.  We review the state of the art attacks and defenses in Section \ref{sec:rw}.

Several software-based defenses have been proposed against Adversarial Machine Learning (AML) attacks~\cite{distillation_SP, nayebi2017biologically, na2017cascade}, but more advanced attack strategies~\cite{CW, DLres} also continue to evolve that demonstrate vulnerability of some of these defenses. Moreover, many of the proposed defenses introduce substantial overheads to either the training or the inference operation of CNNs~\cite{xie2019feature, na2017cascade}.  These overheads increase the computational requirements of these systems, which is already a significant challenge driving substantial research into algorithmic and hardware techniques to improve CNN performance and energy-efficiency~\cite{reviewDL}.    %Another challenge in deploying such systems is their high power and computational requirements, which make them challenging to deploy in embedded systems and latency critical applications. For this reason, many research studies have explored techniques to accelerate CNNs ranging from algorithmic optimizations, hardware acceleration, and even dedicated mobile platforms~\cite{reviewDL}.  Since many of the proposed defenses against adversarial attacks require substantial additional overheads, they make it more challenging to build secure CNNs under power and computational resource constraints.
Thus, finding new approaches to harden systems against AML without heavy overheads in both design-time and run-time is an area of substantial need.

In this paper, we propose a new hardware based approach to improve the robustness of machine learning (ML) classifiers.  Specifically, we show that Approximate Computing (AC),  designed to improve the performance and power consumption of algorithms and processing elements,  can substantially improve CNN robustness to AML.  % AC is a design paradigm that trades precision for power and/or performance gain. 
%Since CNNs are highly tolerant to computational errors \cite{D&T,iccd18}, they represent an ideal candidate for approximate implementation. % AC can reduce the complexity of the expensive multiplication operations, thereby promoting their deployment in energy and resource constrained devices devices.  
%While AC has been explored to reduce power consumption and computation complexity, in this paper, we show for the first time that it can also provide a defense mechanism against adversarial attacks.
Our technique, which we call \emph{defensive approximation} (DA), substantially enhances the robustness of CNNs to adversarial attacks. %Note that, throughout the paper, we refer to classifiers that use DA as approximate classifiers.  
We show that for a variety of attack scenarios, and utilizing a range of algorithms for generating adversarial attacks, DA provides substantial robustness even under the assumptions of a powerful attacker with full access to the internal classifier structure.   Importantly, DA does not require retraining or fine-tuning, allowing pre-trained models to benefit from its robustness and performance advantages by simply replacing the exact multiplier implementations with approximate ones.   The approximate classifier achieves similar accuracy to the exact classifier for Lenet-5 and Alexnet. 

DA also benefits from the conventional advantages of AC, resulting in a less complex design that is both faster and more energy efficient.   Other defenses such as Defensive Quantization (DQ)~\cite{DQ} also provide energy efficiency benefits in addition to robustness.  However, we show that because it is input-dependent DA achieves twice higher robustness to attacks than DQ.
 
%We evaluate DA's robustness properties empirically against several threat models and using a range of adversarial example generation algorithms.  %First, we consider whether an attacker that has access to the exact classifier and generates adversarial examples that fool that classifier, would be able to use those examples against the approximate classifier.  We find that these attacks exhibit poor transferability to the approximate classifier (e.g., over 80\% of Lenet-5 adversarial examples are classified correctly by the approximate classifier). We then consider two scenarios where the attacker directly attacks the approximate classifier:
%\begin{itemize}
%    \item Black-box attack: the attacker reverse engineers the approximate classifier and constructs a proxy of it that uses exact multipliers.  Adversarial examples are generated using this proxy model.  While these examples transfer back to fool the exact classifier, they are not able to fool the approximate classifier.  
%    \item White-box attack: the attacker has full access to the approximate classifier, and can use it to generate examples that reliably fool the approximate classifier.  In this case, we show that the amount of injected noise needed to fool the approximate classifier is substantially higher than the noise needed to fool an exact classifier, for example resulting in around 4db degradation of the adversarial example (and 6x increase in Mean Square Error) for DA relative to the ones that fool the exact classifier. % under $C\&W$ attack, and over $7 dB$ under DeepFool attack.%Nael: perhaps we can make a statement based on the magnitude of the noise.  Also, check the 2db average -- from the figure, it seems higher than that.
%\end{itemize}

We carry out several experiments to better understand the robustness advantages of DA.  We show that the unpredictable and input-dependent variations introduced by AC improve the CNN resilience to adversarial perturbations. Experimental results show that DA has a confidence enhancement impact on non-adversarial examples; we believe that this is due to our AC multiplier which adds input dependent approximation with generally higher magnitude at large multiplication values. In fact, the AC-induced noise in the convolution layer is shown to be higher in absolute value when the input matrix is highly correlated to the convolution filter, and by consequence highlights further the features. This observation at the feature map propagates through the model and results in enhanced classification confidence, i.e., the difference between the $1^{st}$ class and the "runner-up". Intuitively and as shown by prior work~\cite{smooth}, enhancing the confidence furthers the classifier's robustness.% This has also been formally proven in \cite{smooth}. %\nael{Would be good to make the argument about how DA increases the confidence in the classification.  The current paragraph repeats the top level observations about greybox and black box rather than explain.  The last sentence or two explain a bit but would rather focus the whole paragraph on that.} 
%In particular, DA increases the CNN resilience to grey-box adversarial attacks by significantly decreasing the transferability of adversarial examples. It also defends against black-box attacks by making it more difficult to exploit reverse-engineered models for building effective adversarial attacks. %More precisely, an attacker that reverse engineers the classifier and uses the model to generate adversarial examples fails to fool the approximate classifier with high probability. 
%Moreover, DA enhances CNNs resilience to white-box attacks by making the generation of adversarial examples process more challenging; Generating adversarial examples under white-box setting requires high perturbations' amplitude, thereby undermining the very concept of adversarial noise imperceptibility. 
At the same time, we observe negligible accuracy loss compared to a conventional CNN implementation on non-adversarial inputs while providing considerable power savings.  

%We show that the robustness advantages of DA arise from the data dependent approximate multiplier design that we use.  By implementing approximate multipliers instead of conventional ones, we build approximate convolution layers that, by-design, inject additive data-dependent noise into the process. %The approximation is designed such as the AC-induced noise is input-dependent. 
%We show empirically that this property helps the convolution capture the important features more efficiently, thereby enhancing classification confidence, and making it more difficult (i.e., it requires more noise) to cause the approximate model to misclassify.  \nael{Not sure that we established the data dependent part as necessary}

%%
  %Related to our work, a set of defenses based on randomization emerged over the last years, and provide theoretically quantifiable robustness bounds~\cite{smooth,snP2019_certif,defense_certified}.  Unlike our implementation, these works assume introduction of Gaussian noise at different stages of the operation of the classifier; our approximate multiplier is sensitive to the input data, but is not Gaussian.   However, these works support our general observation that the injection of perturbations improves the robustness of the classifier.  From a practical perspective, none of these works have been evaluated at scale or with realistic implementations.  For example, Raghunathan et al.~\cite{defense_certified} evaluate only a tiny neural network.  Other works~\cite{smooth,snP2019_certif} consider scalability but require high overhead to implement the defense. Specifically, to estimate the model output, %. In fact, the scores and labels are estimated by these methods require running  a  heavy  Monte  Carlo  simulation involving a number of different runs of the CNN for the same input.
%Our approach is different since, not only our AC-injected noise does not require overhead but comes naturally from the simpler and faster AC implementation. Moreover, while these techniques require additional training, our implementation is a drop-in replacement of the hardware without specific training requirements, and with no changes to the architecture nor the parameters of the CNN.   
%%
%In fact, the approximate classifier is around 4x faster than the exact classifier, and 2.5x more energy efficient.  %\nael{Should focus this paragraph mostly on the security properties -- the overhead is the secondary argument.}

%For  example,  Raghunathan  et  al.  [15]evaluate  only  a  tiny  neural  network.  Other  works  [13],  [14]consider  scalability  but  require  high  overhead  to  implementthe defense. Specifically, to estimate the model output whichrequires  running  a  heavy  Monte  Carlo  simulation  involvinga  number  of  different  runs  of  the  CNN  for  the  same  input.Our  approach  is  different  since,  not  only  our  AC-injectednoise does not require overhead but comes naturally from thesimpler and faster AC implementation. Moreover, while thesetechniques require additional training, our implementation is adrop-in replacement of the hardware without specific trainingrequirements, and with no changes to the architecture nor theparameters of the CNN. In fact, the AC classifier is around 4xfaster than the exact classifier, and 2.5x more energy efficient.In summary, the contributions of the paper are


In summary, the contributions of the paper are:
\begin{itemize}
    \item We build an aggressively approximate floating point multiplier that injects data-dependent noise within the convolution calculation. Subsequently, we used this approximate multiplier to implement an approximate CNN hardware accelerator (Section \ref{sec:AppxCNN}).  %\nael{This is the first time we mention Ax-FPM.  Probably introduce it earlier in the intro and explain why it is a good choice.}
    \item To the best of our knowledge, we are the first to leverage AC to enhance CNN robustness to adversarial attacks without the need for re-training, fine-tuning, nor input pre-processing. We investigate the capacity of AC to help defending against adversarial attacks in Section \ref{sec:secu}.
    \item We empirically show that the proposed approximate implementation reduces the success rate of adversarial attacks by an average of 87\% and 71.5\% in Lenet-5 and Alexnet CNNs respectively.% and 87.5\% in Lenet-5 for  black-box attacks.
    \item We evaluate the approximate classifiers against powerful attackers with white-box access.  We observe that attackers require substantially higher adversarial perturbations to fool the approximate classifier.
    %\item We provide a theoretical analysis to gain insights into processes that allow DA to improve robustness  (Appendix \ref{sec:theory}). 
    
    %\nael{Anything to say about black box attacks?} \ihsen{done.}
    %\item We demonstrate that the security enhancement property comes with no cost in terms of accuracy and classification performance. % even aggressive approximation can be tolerated by CNNs (maintaining accuracy) %thereby obfuscating the use of circuit-level approximations to a potential attacker.

    %\nael{Do we want to say anything about the effect of improving accuracy?} \ihsen{Overall, AC improves confidence (scores), but not necessarily accuracy overall.}
    %\item We show that data-dependent approximation helps with carrying useful information and thereby smoothing the shape of the decision boundary.
    %\item We make our scripts publicly available for the community. 
\end{itemize}

\noindent 
We believe that DA is highly practical; it can be deployed without retraining or fine-tuning, achieving comparable classification performance to exact classifiers.  In addition to security advantages, DA {\em improves} performance by reducing latency and energy making it an attractive choice even in Edge device settings (Appendix \ref{sec:perf_impl}).



==> asplos21main-p898-p (Copy)/Performance_implications.tex <==
\subsection{Impact on Model Accuracy} %(a) same data distribution (b) noise }
\label{CNNaccuracy}
%It seems pointless to use a defense mechanism that degrades the model's accuracy on clean data: taking the risk of affecting the actual task of a model to avoid attacks, especially if these attacks have a low probability or a low impact on the system, it is then unacceptable to tolerate a decrease in the clean data accuracy.
It is important for a defense mechanism that aims to enhance robustness against adversarial attacks to keep at least an acceptable performance level for clean inputs. In fact, considerably reducing the baseline accuracy, or creating an exploding or vanishing gradient impact that makes the model sensitive to other types of noise undermines the model reliability.  
In our proposed approach, we maintain the same level of recognition rate even with the approximate noise in the calculations. Counter-intuitively, this data-dependent noise helps to better highlight the input's important features used in the recognition and does not affect the classification process. 
%confirming the inherent error-resiliency of CNNs. 
A drop of $0.01 \%$ in the recognition rate for the case of LeNet-5 and $1\%$ for AlexNet is recorded as mentioned in Table \ref{tab3}. 

%\begin{table}[!htp]
%\small
%\centering
%  \caption{Accuracy results of the LeNet-5 and AlexNet CNNs.}
%  \label{tab3}
%  \begin{tabular}{ccc}
%    \toprule
%    \textbf{Used Multiplier }& \textbf{LeNet5} & \textbf{AlexNet}\\
%    \midrule
%        Exact multiplier        & 97.93\%  &   81\%   \\
     %   HEAP                    &  97.86\% &    80.65\%       \\
%        Ax-FPM	                & 97.67\%  &   80\%     \\ 
%  \bottomrule
%\end{tabular}
%\end{table}

\begin{table}[!htp]
\small
\centering
  \caption{Accuracy results of Float32, approximate model, fully quantized, weight-only quantized and Bfloat16 models.}
  \label{tab3}
  \begin{tabular}{ccc}
    \toprule
    \textbf{Used Multiplier }& \textbf{MNIST} & \textbf{CIFAR-10}\\
    \midrule
        Float32                 & 97.93\%  &   81\%   \\
     %   HEAP                   &  97.86\% &    80.65\%  \\
        Approximate (DA)	    & 97.67\%  &   80\%     \\ 
        Fully quantized         & -     &   80\%  \\
        Weight-only quantized   & -     &  80\% \\
        Bfloat16                & 97.93  &  81\% \\
        
  \bottomrule
\end{tabular}
\end{table}

%\subsection{Defensive approximation and sensitivity}

%To further investigate the stability of the approximate classifier, we explored the inference results under input random perturbation. In Table \ref{gaussianNoise}, random Gaussian noise ($mu = 0$, $std = 0.01, 0.05, 0.1$) was added to the input images and fed to both exact and approximate model in order to evaluate their sensitivity to random white noise (Note that noise added to a grey-scaled input image with a standard deviation equal to 0.1 is considered as aggressive noise). Measuring the accuracy of both classifiers, we notice that the approximate classifier is more robust to white Gaussian noise, and this could be explained by the fact that the introduced approximation is pushing the decision boundary further from the input image making it harder for this input to cross the boundary. Our proposed approximate classifier is not only resilient to adversarial perturbations but also to white Gaussian noise.   %see reviewer comment

%\begin{table}[!htp]
%\centering
%  \caption{Accuracy results when adding Gaussian noise to input images from the MNIST dataset.}
%  \label{gaussianNoise}
%  \begin{tabular}{cccc}
%    \toprule
%    \textbf{Classifier }& \textbf{ std = 0.01}& \textbf{std = 0.05} & \textbf{std = 0.1}\\
%    \midrule
%        Exact      &  96\%  &   95.5\%   &   93\%   \\
%        Approximate	&   96\% &  95.5\%    &   94\%     \\ 
%  \bottomrule
%\end{tabular}
%\end{table}

\subsection{Impact on Performance and Energy Consumption}

% %\begin{figure}[!tp]
% %\centering
% %\includegraphics[width=0.85\columnwidth]{asplos21-templates/delay_energy.pdf}
% %,height=5cm
% %\caption{Energy, delay and EDP of AMA5-based $24\times24$ approximate multiplier normalized to a conventional multiplier.}
% %\label{fig:energy}
% %\end{figure}

% \sout{

Here we show the additional benefit of using AC, especially in the context of power-limited devices, such as mobile, embedded, and Edge devices.
The experiments evaluate normalized energy and delay achieved by the proposed approximate multiplier compared to a conventional baseline multiplier. Multipliers are implemented using $45~ n m$ technology via the Predictive Technology Model (PTM) using the Keysight Advanced Design System (ADS) simulation platform~\cite{PTM}.  
% }

 \begin{table}[!htp]
 \centering
   \caption{Energy and delay Comparison.}
   \label{tab:energy}
   \begin{tabular}{ccc}
     \toprule
     \textbf{Multiplier }& \textbf{Average energy}	& \textbf{Average delay}  	 \\
     \midrule
         Exact multiplier        & 1 & 1    \\
         %HEAP                   & 0.49  & 0.46\\
         %Ax-FPM	             & 0.501 & 0.328\\ 
         Ax-FPM	                 & 0.487 & 0.29\\ 
         Bfloat16                & 0.4   & 0.4   \\
   \bottomrule
 \end{tabular}
 \end{table}
 
% \sout{
Table \ref{tab:energy} compares the energy and delay for the approximate multiplier and the Bfloat16 multiplier normalized to a conventional multiplier. 
\begin{figure}[!htp]
\centering
\includegraphics[width=1\columnwidth]{32fp_16bf.PNG}
\caption{Contrast between IEEE 754 Single-precision 32-bit floating-point format and Bfloat16 format.
}
\label{fig:bfloat}
\end{figure}

Bfloat16 data representation is shown in Figure \ref{fig:bfloat}, with 1 sign bit, a 8-bit exponent and a 7-bit fraction. The used Bfloat16 multiplier has similar architecture to that of Ax-FPM. However for the mantissa multiplier we use the conventional Booth multiplier instead of the array multiplier.
Ax-FPM achieves up to $51\%$ and $71$\% savings in energy and delay, respectively compared to the baseline multiplier. Bfloat16 implementation results in comparable savings with around $60\%$ lower power and delay. However, this comes without robustness advantages, as mentioned earlier.

 %60\% of exact mantissa multiplier total consumption, adding the power gained by eliminating the rounding unit, the final power saving of the whole FPM exceeds 67\%.
 %The approximate circuit also achieves more than $60\%$ reduction in delay.  AMA5 uses only eight transistors rather than 28; corresponds to 72\% area savings. %
 Unlike most of the state-of-the-art defense strategies that lead to power, resource, or timing overhead, DA results in saving energy and area.
% }


==> asplos21main-p898-p (Copy)/Proposed_approach.tex <==
%\subsection{Approximate CNN}

We propose to leverage approximate computing to improve the robustness of ML classifiers, such as CNNs, against adversarial attacks. We call this general approach \textbf{Defensive Approximation} (DA). The closest approach to DA is the perturbation-based defense~\cite{snP2019_certif,smooth} that either adds noise or otherwise filter the input data to try to interfere with any adversarial modifications to the input of a classifier. However, our approach advances the state-of-the-art by injecting perturbations throughout the classifier and directly by the approximate hardware, thereby enhancing both robustness and power efficiency. 

Technically, the approximate design process is driven by two main considerations:
\begin{enumerate}[label=(\alph*)]
    \item Injecting significant noise that can influence the CNN behavior, and allows by-product power gains. %This led us to choose an aggressively approximate multiplier to be deployed.
    \item Keeping the cumulative noise magnitude under control to avoid impacting the baseline accuracy of the CNN. %For this reason, we purpose to change the mantissa multiplier only (fraction), while keeping the exponent part unchanged (exact).
\end{enumerate}

For consideration (b), we purpose to an implementation that replaces the conventional mantissa multiplier in floating point multipliers, with a simpler approximate design. This choice is backed by the study in \cite{iccd18, D&T}, which show that errors in the exponent part might have a drastic impact on CNNs accuracy. 
Consideration (a) means that the approximate design needs to be aggressive to induce significant noise. Therefore, as detailed in the next subsection, we chose the corner case, i.e., the most aggressive approximate design \cite{AMA5, Heap}, and used it to replace the mantissa computation logic in a basic floating point multiplier. %Moreover, for the sake of comparison, we also proceed to a design space exploration and compare our design to a less aggressive approximate design \cite{Heap}.} 



In this section, we present our approximate multiplier design and analyze its properties.
%\nael{I think this opens a door for the reviewers to question our time and power analysis.   Are you evaluating the mantissa manipulation and the rounding logic in the power and latency analysis?} \ihsen{The power and delay analysis is for the Mantissa Multiplier, and I think I can have numbers for the whole FP multiplier.}

\subsection{Approximate Floating Point Multiplier}
%\textcolor{blue}{Khaled: we do not discuss HEAP anywhere in this subsection}
ML structures, such as CNNs, often rely on computationally expensive operations, e.g., convolutions that are composed of multiplications and additions. Floating-point multiplications consume most of the processing energy in both inference and training of CNNs~\cite{esl_ihsen,Heap}. %\nael{Note missing citation} \amira{@Ihsen I think you have a paper where u proved that we can cite it}
Although approximate computation can be introduced in different ways (with likely different robustness benefits), DA leverages a new approximate 32-bit floating-point multiplier, which we call \textit{approximate floating-point multiplier} (Ax-FPM).
The IEEE 754-2008 compliant floating-point format binary numbers are composed of three parts: a sign, an exponent, and a mantissa (also called fraction)~\cite{FP}. %\nael{note missing citation} 
The sign is the most significant bit, indicating whether the number is positive or negative. In a single-precision format, the following $8$ bits represent the exponent of the binary number ranging from $-126$ to $127$. The remaining $23$ bits represent the fractional part (mantissa). 
For most of the floating number range, the normalized format is:
\begin{equation}\label{eqn:ieee754}
val = ( -1 )^{\textit{sign}} \times 2^{exp-bias} \times ( 1.fraction ) 
\end{equation}

A floating-point multiplier (FPM) consists mainly of three units: mantissa multiplier, exponent adder, and a rounding unit.  The mantissa multiplication consumes $81\%$ of the overall power of the multiplier \cite{trunca}.% We choose to approximate the mantissa multiplication unit only for two main reasons: \textbf{(i)} Approximating the mantissa prevents massive noise injection that can result from perturbing the exponent or sign, and \textbf{(ii)} The mantissa multiplication consumes $81\%$ of the overall power of the multiplier \cite{trunca}.

Ax-FPM is designed based on a mantissa multiplication unit that is constructed using approximate full adders (FA). The FAs are aggressively approximated to inject computational noise within the circuit. We describe Ax-FPM by first presenting the approximate FA design, and then the approximate mantissa multiplier used to build the Ax-FPM. 
%We used implementation of an approximate mirror adder as a building block of the $24 \times 24$ mantissa multiplier.
%This latter provides a reduction in power consumption and resource utilization, as well as an increase in processing speed while introducing some calculation errors.

%\vspace{-6pt}
%\subsection{Approximate Floating Point multiplier (Ax-FPM)}

% (RU, which accounts for $18\%$ of the power). We also eliminate the RU resulting in further approximation when rounding is needed.

\begin{figure}[!htp]
\centering
\includegraphics[width=\columnwidth]{Mantissa_multiplier0.pdf}
\caption{An illustration of a $4 \times 4$ array multiplier architecture.}
\label{MA}
\end{figure}

To build a power-efficient and a higher performance FPM, we propose to replace the mantissa multiplier by an approximate mantissa multiplier; an array multiplier constructed using approximate FAs. We selected an array multiplier implementation because it is considered one of the most power-efficient among conventional multiplier architectures~\cite{array}.  In the array architecture, multiplication is implemented through the addition of partial products generated by multiplying the multiplicand with each bit of multiplier using AND gates, as shown in Figure \ref{MA}.  %In the case of a 32-bit floating-point multiplier, the mantissa multiplication is a $24\times24$-bit multiplication. %The exact full adder was replaced by an approximate mirror adder (AMA5). 
\begin{figure}[!htp]
\centering
\includegraphics[width=\columnwidth]{full_adder.pdf}
\caption{Logic diagram of (a) exact Full Adder, (b) AMA5 (used in this work).}
\label{FA}
\end{figure}

Specifically, we build an array multiplier based on an approximate mirror adder (AMA5)~\cite{AMA5} in place of exact FAs. The approximation of a conventional FA is performed by removing some internal circuitry, thereby resulting in power and resource reduction at the cost of introducing errors.  Consider a FA with (A,B, $C_{in}$) as inputs and ($Sum$, $C_{out}$) as outputs ($C$ here refers to carry). For any input combination, the logical \textit{approximate} expressions for $Sum$ and $C_{out}$ are: $Sum = B$ and $C_{out} = A$. %as shown in Table \ref{tab1}.
%\textcolor{blue}{khaled: the table is missing are we removing it?}  %Notice that the two outputs are input-dependent, 
%\textcolor{red}{Amira: I did to gain some space, I thought this committee is probably aware of this appx mirror adder.}\textcolor{blue}{khaled: if possible, you can add citation instead}
The AMA5 design is constituted by only two buffers (see Figure \ref{FA}), leading to the latency and energy savings relative to the exact design, but more importantly, introduce errors into the computation.  It is worth noting that these errors are data dependent, appearing for specific combinations of the inputs, and ignoring the carry in value, making the injected noise difficult to predict or model.  %This approximation leads to a low-power and low-area design compared to a conventional FA. 

%\begin{table}[!htp]
%\small
%\centering
%  \caption{Truth Tables of Exact FA and AMA5.}
%  \label{tab1}
%  \begin{tabular}{|c|c|c|c|c|c|c|}
%    \toprule
%\multicolumn{3}{|c|}{\textbf{Inputs}}	& \multicolumn{2}{|c|}{\textbf{Exact}}	%& \multicolumn{2}{|c|}{\textbf{AMA5}}  \\
%\hline
%\textbf{$A$ }	& \textbf{$B$}	& \textbf{$C_{in}$}  & \textbf{$Sum$} & %\textbf{$C_{out}$}& \textbf{$Sum$} & \textbf{$C_{out}$} \\
%    \midrule
%        0	& 0 & 0	& 0 & 0 & 0 & 0\\
%        0	& 0	& 1	& 1 & 0 & 0 & 0\\
%        0	& 1	& 0	& 1 & 0 & 1 & 0\\
%        0   & 1	& 1	& 0 & 1 & 1 & 0\\
%        1   & 0 & 0	& 1 & 0 & 0 & 1\\
%        1   & 0 & 1 & 0 & 1 & 0 & 1\\
%        1   & 1 & 0 & 0 & 1 & 1 & 1\\
%        1   & 1 & 1	& 1 & 1 & 1 & 1\\

%  \bottomrule
%\end{tabular}
%\end{table}

%To assess the accuracy of the approximate FP multipliers, these latter were designed and a behavioral simulation was performed. The baseline performance of the isolated approximate multipliers were evaluated using one million products of randomly generated FP values. The accuracy results in the level is expressed in terms of the mean error distance (MED), the mean relative error distance (MRED) and the normalized mean error distance (NMED), which are metrics commonly used to compare approximate circuits and track error propagation \cite{metrics}:
%\begin{equation}
%    MED = \frac{1}{n} \sum_{i=1}^{n} \mid{ Y^{*} -Y}\mid
%\end{equation}

%\begin{equation}
%    MRED= \frac{1}{n} \sum_{i=1}^{n} \frac{ \mid{ Y^{*} -Y}\mid}{Y}
%\end{equation}

%\begin{equation}
%    NMED= \frac{1}{n} \sum_{i=1}^{n} \frac{ \mid{ Y^{*} -Y}\mid}{P_{max}}
%\end{equation}

%Where $Y$ is the exact result, $  Y^{*} $ is the approximate result, and $P_{max}$ is the maximum product.

%The accuracy results are reported in Table \ref{tab4}. For one million multiplication of inputs ranging between $10^{-4}$ and $1$, we


%The impact of the approximation multiplier is in the order of $10^{-6}$ in the NMED for the case of Ax-FPM and $10^{-7}$ for HEAP, which is consistent with previously introduced state-of-the-art approximate multipliers \cite{AppxMult}.

%\begin{table}[!htp]
%\centering
%  \caption{Accuracy results of different multipliers.}
%  \label{tab4}
%  \begin{tabular}{cccc}
%    \toprule
%    \textbf{Multiplier } & \textbf{MED} & \textbf{MRED} & \textbf{NMED}	 \\
%    \midrule
%        Exact multiplier &  0   & 0  & 0        \\
%        Ax-FPM	         &  4.95    &  457.20  & 2.47  \\ 
%  \bottomrule
%\end{tabular}
%\end{table}
%%%

%Analyze the performance of the multiplier

When trying to evaluate the proposed Ax-FPM, we were interested in studying its behavior under small input numbers ranging between $-1$ and $+1$ since most of the internal operations within CNNs are in this range. %To assess the accuracy of the approximate FP multiplier, this latter was designed and a behavioral simulation was performed. 
%We also tested an implementation using a more accurate approximate multiplier called heterogeneous approximate floating-point multiplier (HEAP) \cite{Heap}. HEAP is the result of a design space exploration among combinations of different approximate full adders leading to minimal accuracy loss.

We measure the introduced error as the difference of the output of the approximate multiplier and the exact multiplier. The results are shown in Figure \ref{appx_mult} using 100 million randomly generated multiplications across the input range from $-1$ to $1$. 
\begin{figure}[!htp]
\centering
\includegraphics[width=0.8\columnwidth]{error_dist_axfpm.pdf}
\caption{Noise introduced by the approximate multiplier while the operands in $[0,1]$.
}
\label{appx_mult}
\end{figure}
Three trends can be observed that will be used later to help understanding the impact of the approximation using Ax-FPM on CNN security: \textbf{(i)} The first is the data-dependent discontinuity of the approximation-induced errors, \textbf{(ii)}  We noticed that in $96\%$ of the cases, the approximate multiplication results in higher absolute values than the exact multiplication: For positive products, the approximate result is higher than the exact result, and for negative product results the approximate result is lower than the exact result, and \textbf{(iii)} In general, we notice that the larger the multiplied numbers, the larger the error magnitude added to the approximate result. As shown later, these observations will help understand the mechanism that we think is behind robustness enhancement. 

\begin{figure}[!htp]
\centering
\includegraphics[width=0.9\columnwidth,height=4cm]{Convolution.pptx.pdf}
\caption{Convolution result of the filter and each input image using exact and approximate convolution.}
\label{appx_conv}
\end{figure}

\subsection{Approximate Convolution}

In order to understand the impact of AC at larger scales than the individual multiplication, we track the impact on convolution operations. The approximate CNN is built using the approximate convolution operations as building blocks. The activation functions and the pooling layers which do not use multiplication are similar to the conventional CNN.   Convolution layers enable CNNs to extract data-driven features rather than relying on manual feature-extraction in classical ML systems. The convolution operation is performed on the layer's input data using a kernel matrix that is convoluted (piece-wise multiplied) against the input data to produce a feature map. %The convolution is executed by sliding the kernel over the input. 
%At every receptive field, a matrix multiplication is performed and the result is summed onto the feature map as shown in Figure \ref{conv}. 
%Specifically, the output of each convolution operation is the dot product of the input matrix $I$ and a weight kernel $W$ % The convolution is then expressed by $Conv(I,W) = \sum I_{ij}* W_{ij}$. 
%computed as follows:

%\begin{equation}
%\label{eq:convlayer}
%O[x][y] = B + \sum_{i=0}^{R-1} \sum_{j=0}^{R-1} I[S_x+i][S_y+j] \times W[i][j]
%\end{equation}

%where $O$ is the output feature map, $B$ is the bias vector, $R$ is the size of the kernel, and $S$ is the stride.

As we slide the filter over the input from left to right and top to bottom whenever the filter coincides with a \textbf{similar} portion of the input, the convolution result is high, and the neuron will fire. %For all other parts of the input image that doesn’t align with the filter, the output will be lower. 
The weight matrix filters out portions of the input image that does not align with the filter, and the approximate multiplier helps improve this process by further increasing the output when a feature is detected. In Figure \ref{appx_conv}, we run an experiment where we choose a filter and six different images with different degrees of similarity to the chosen filter (1 to 6 from the least to the most similar), and we perform the convolution operation. We notice that the approximate convolution using Ax-FPM delivers higher results for similar inputs and lower results for dissimilar inputs. We can also notice that the higher the similarity, the higher the gap between the exact and Ax-FPM approximation results.  Therefore, by using the approximate convolution, the main features of the image that are important in the image recognition are retained and further highlighted with higher scores that will later help increase the confidence of the classification result, as explained in Section \ref{sec:how}.

%\textcolor{blue}{In contrast, We notice that the approximate convolution \textcolor{blue}{using HEAP} delivers similar results to the exact multiplier implantation for both similar inputs and dissimilar inputs.}

% \begin{figure}[!htp]
% \centering
% \includegraphics[width=\columnwidth]{error_dist.pdf}
% \caption{Error distribution of an approximate convolution.}
% \label{error_dist}
% \end{figure} 
%\subsection{Approximate CNN}

%\nael{Is the next paragraph included here by mistake from a previous version?  It seems to go back to the analysis of the multiplier noise.  Not sure if it can be merged with the earlier text or eliminated.}
%To track the impact of the approximation on the convolution layer, we replace the exact multiplication with the approximate one.
%Several convolution operations for random inputs ranging between $-1$ and $1$ were performed using exact and approximate multipliers and their outputs were collected and examined. We set the error as the difference between the approximate output and the exact output. Measuring the probability distribution function of the error between the exact and the approximate output of the convolution layer we found that the error caused by Ax-FPM is normally distributed. Errors near the $ mean = 0.01$ are more frequently occurring with a standard deviation of $std = 0.39$. %, see Figure \ref{error_dist}.



% For the sake of the illustration, in Figure \ref{appx_cnn} we present an end-to-end CNN toy example for horizontal edge detection in which we show the effect of approximation on the model output. We can see that, while both exact and approximate implementations correctly classify the input, the score of the class \emph{"Horizontal"} is higher in the approximate implementation. This illustration shows that the convolution-extracted features enhancement due to the approximate multiplier propagates to the output thereby enhancing the CNN confidence. This aspect will be further investigated in Section \ref{subsec:confidence}.

% \begin{figure*}[!htp]
% \centering
% \includegraphics[width=2\columnwidth]{endtoendcnn.pdf}
% \caption{End to End simple exact and approximate CNN examples for horizontal edge detection. \ihsen{Not sure if this figure needs to stay: does it help understand? Or does it over simplify, at the risk of devaluing the idea?}}
% \label{appx_cnn}
% \end{figure*}



\subsection{AC Design Space Exploration}
For the sake of comparison, we proceed to a design space exploration considering the accuracy of the multipliers and resource utilization as optimization objectives. The comparison of our design with the optimal approximate design given by the exploration and referred to as HEAP led to a clearly dominant choice in favor of our design given the following perspectives:
%this subsection, we address the choice of the approximate multiplier design. During a multi-objective design space exploration considering multipliers' accuracy and resource utilization led to the following observations:



\textbf{(i) Resource and power efficiency:} Given its aggressive design, Ax-FPM achieves the lowest power consumption and resource utilization. %Comparative results with HEAP are given in Figure \ref{fig:energy}. 

\textbf{(ii) Robustness:} While other approximate designs had a positive impact on CNNs robustness, we noticed that Ax-FPM achieves the highest enhancement. 

\textbf{(iii) Accuracy:} CNNs are highly approximation-tolerant, and even aggressive multiplier design didn't impact overall accuracy. Ax-FPM, as well as HEAP have insignificant impact on accuracy. %Comparative results are shown later in Table \ref{tab3}.

While these observations give an insight on the potential generalizability of AC positive impact, Ax-FPM is a non dominated design outperforming other design in both robustness, power consumption and resource utilization, while having the same overall accuracy level. 
Hence, in the remainder of the paper, we will focus only on Ax-FPM based DA. Further details and results can be found in the Appendix.


==> asplos21main-p898-p (Copy)/Quantization.tex <==

In this section, we investigate the impact of other reduced precision techniques on robustness. We first compare DA to DQ, and then study the impact of using Bfloat16 data representation on the system performance and robustness.

%\label{sec:quan}
\subsection{Defensive Quantization}
%Defensive quantization \cite{lin2019defensive} 

Defensive quantization \cite{DQ} was proposed to jointly optimize the efficiency and robustness of deep learning models. A 4-bit quantized model was trained on CIFAR-10 using the Dorefa-Net method \cite{zhou2018dorefanet}. The model architecture is detailed in Appendix \ref{mod_archi}. We consider two ways of quantization: (i) Weight quantization, where only the weights are quantized, and (ii) Full quantization where the weights %\ihsen{CNN input? no?} 
of each convolutional and dense block and the output of each activation function are quantized. %%%%%%%%%%
In Table \ref{quan_result4}, we report transferability between exact (32-bit floating point), approximate model (using DA), fully quantized and weight-only quantized model.
We notice that DA is almost  two times more robust against transferability attacks than DQ under FGSM, PGD and C\&W attacks. We believe that this is due to the difference in terms of noise distribution between DA and DQ. In fact, while DQ-induced noise tends to make the initial decision boundary smoother, the input-dependent noise in DA makes its decision boundary randomly different from the initial model.

\begin{table}[!htp]
\small
  \caption{Comparing attacks transferability success rates for CIFAR-10 when using DA and DQ.}
  \label{quan_result4}
  \begin{tabular}{ccccc}
    \toprule
                     &          & \textbf{DA:} & \textbf{DQ:} & \textbf{DQ:} \\
    \textbf{Attack method} & \textbf{Exact}  &  & \textbf{Full } & \textbf{Weight-only } \\
    \midrule
        FGSM          &   100\%    & 38\%  & 60\%  & 61\% \\
        PGD           &   100\%    & 31\%  & 74\% & 73\%\\
        C\&W          &   100\%    & 17\%  & 68\% &  68\% \\
        
  \bottomrule
\end{tabular}
\end{table}

\subsection{BFloat16}

The Bfloat16 (Brain Floating Point) \cite{ kalamkar2019study} is a truncated version of the 32-bit IEEE 754  single-precision floating-point format (float32). It is composed of one sign bit, eight exponent bits, and seven mantissa bits giving the range of a full 32-bit number but in the data size of a 16-bit number. Bfloat16 is used in machine learning applications and intended to reduce the storage requirements and increase computing speed without losing precision. 

To evaluate the impact of Bfloat16 on deep neural networks robustness, we use Pytorch framework \cite{PyTorch} to implement Bfloat16-based CNN architectures and test them for MNIST and CIFAR-10 benchmarks.
We notice that using Bfloat16 achieves the same prediction accuracy as the full precision 32-bit floating point. No remarkable change was noticed at the output of the convolutional layers nor in the confidence of the models. We believe this is due to the nature of the noise introduced by reducing data representation accuracy. A more detailed discussion can be found in Section \ref{discussion}. 

Figure \ref{bfloat16} shows the noise resulting from multiplying $100$ million randomly generated Bfloat16 numbers compared to their corresponding 32-bit floating point. This figure shows that, in contrast with our approximate multiplier (Figure \ref{appx_mult}), Bfloat16 multiplication results in mostly negative noise with orders of magnitude lower than DA-induced noise. Moreover, the Bfloat16 noise is not input-dependent, and has no specific impact on the model confidence. Accordingly, no improvement in the robustness was noticed when attacking the Bfloat16 model using FGSM, PGD and $C\&W$. 

\begin{figure}[!htp]
\centering
\includegraphics[width=0.9\columnwidth]{error_dis_bfloat16.pdf}
\caption{Noise introduced by multiplying Bfloat16 while the operands $\in [0,1]$.
}
\label{bfloat16}
\end{figure}




==> asplos21main-p898-p (Copy)/Related_work.tex <==
%\textbf{Approximate computing.} Motivated by reducing the overhead of CNNs, three main approximation levels have been studied in the literature. The first reduces the precision of operands through a quantization process of the parameters. It usually consists of converting values from floating point to an N-bit fixed point number \cite{survey_121}, \cite{survey_122}. %%Authors in \cite{survey_121} reduce the weights bitwidth to 8 bits and the activation to 10. In \cite{survey_122}, both weights and activation can reach 8-bits with fine-tuning. 
%In \cite{survey_127}, authors manage to aggressively reduce the data bit-width. By introducing the concept of binary weights ($-1$ and $1$), the multiply operation is reduced to addition and subtraction only. The same idea is extended in \cite{survey_128} by using binary parameters, thereby reducing the MAC operation to an XNOR. However, these two approaches have a dramatic accuracy loss of $19\%$ and $29.8\%$, respectively \cite{survey_129}. While these works rely on linear quantization with uniformly spaced out values, the weights and activation distributions are not uniform \cite{survey_118,survey_135}. %For example, in \cite{survey_122,survey_135}, weights are quantized to powers of two. Consequently, the multiply operation is substituted by a bitshift operation.
%The second main approximation level is the model-oriented approximations such as compression, pruning, and compact network architectures \cite{survey_94}, \cite{survey_138}. %The sparsity of the rectified linear unit (ReLU) output activation is exploited in \cite{survey_94} to reduce memory access, particularly to costly off-chip memory access. The proposed reconfigurable hardware skips reading the weights and performing the MAC for zero-valued activation thereby reducing energy cost by $45\%$. Authors in \cite{survey_138} go even further and instead of just gating the read and MAC operation, they suggest to skip the cycle to increase the throughput by $1.37 \times$. 
%Networks are usually over-parameterized and a large amount of redundancy exists within their weights. Network pruning techniques such those proposed in \cite{survey_141} aim at removing the redundancy. To maintain the primary accuracy level, aggressive network pruning techniques may require weights fine-tuning.
%These techniques are effective in reducing CNNs size and complexity. However, since the used platforms are at a high abstraction level, they fail to consider circuit-level characteristics. In this context, there are comparatively few studies that propose a fine-grained circuit-level approximation. In this work, we explore gate-level approximation since it provides the highest design flexibility \cite{Heap}.

%\textbf{Defense strategies.} 
Several defense mechanisms were proposed to combat adversarial attacks and can be categorized as follows:



\noindent
\textbf{Adversarial Training (AT).} 
AT is one of the most explored defenses against adversarial attacks. The main idea can be traced back to \cite{fgsm}, in which models were hardened by including adversarial examples in the training data set of the model. As a result, the trained model classifies evasive samples with higher accuracy. Various attempts to combine AT with other methods have resulted in better defense approaches such as cascade adversarial training \cite{na2017cascade}, principled training \cite{certifying}. Nonetheless, AT is not effective when the attacker uses a different attack strategy than the one used to train the model~\cite{samangouei2018defense}. Moreover, adversarial training is much more computationally intensive than training a model on the training data set only because generating evasive samples needs more computation and model fitting is more challenging (takes more epochs)~\cite{tramer2017ensemble}.

%Training on fast non-iterative attacks such as FGSM only results in robustness against non-iterative attacks. 
%Moreover, adversarial training is very computationally intensive, because generating adversarial samples needs more computation and model fitting. 


\noindent
\textbf{Input Preprocessing (IP).}
Input preprocessing depends on applying transformations to the input to remove the adversarial perturbations~\cite{das2017keeping, osadchy2017no}. Examples of transformation are denoising auto-encoders~\cite{gu2014towards}, the median, averaging, and Gaussian low-pass filters~\cite{osadchy2017no}, and JPEG compression~\cite{das2017keeping}. However, it was shown that these defenses are insecure under strong white-box attacks~\cite{chen2019towards}; if the attacker knows the specific used transformation, it can be taken into account when creating the attack. Furthermore, preprocessing requires additional computation on every input. 

%Image transformations such as random resizing and random padding of input image \cite{randomization}, image cropping and re-scaling, bit-depth reduction, JPEG compression, and image quilting \cite{Transformations} all used in an attempt to break the specific structure of the added adversarial perturbation. The problem with transformation-based defenses is that they cause obfuscated gradients which gives a false sense of security \cite{Obfuscated} making the model more sensitive and less reliable.

\noindent
\textbf{Gradient Masking (GM).}
GM relies on applying regularization to the model to make its output less sensitive to input perturbations. Papernot et al. proposed defensive distillation~\cite{distillation_SP}, which is based on increasing the generalization of the model by distilling knowledge out of a large model to train a compact model. Nonetheless, distillation was found weak against $C\&W$ attack \cite{CW}. Nayebi and Surya~\cite{nayebi2017biologically} purposed to use saturating networks that use a loss function that promotes the activations to be in their saturating regime. \cite{ross2018improving} proposed to regularize the gradient input by penalizing variations in the model's output with respect to changes in the input during the training of differentiable models. Nonetheless, GM approaches found to make white-box attacks harder and vulnerable against black-box attacks~\cite{papernot2017practical,tramer2017ensemble}. Furthermore, they require re-training of pre-trained networks. 

%Introducing randomization at different levels (e.g., input data, layers...) \cite{stoch_prunning}, \cite{random} in order to improve the adversarial robustness. It was observed empirically that the randomization-based defenses help in smoothing the prediction function, hence increase its resilience to adversarial noise. The drawback is that these defenses does not provide a design guideline on the amount of noise that should be injected or its location

%A defense mechanism called \textit{Pixel}DP based on Differential Privacy \cite{snP2019_certif} included in the learning procedure to increase the model robustness to adversarial examples. This technique lead to an impractical prediction procedure: using a Monte Carlo method to approximate the model prediction.

%Adversarial training was suggested in \cite{goodfellow2014b} where the adversarial examples are constantly updated during the training process. This technique was proven to be inefficient since new adversarial examples still can fool the network. Various attempts to combine adversarial training with other methods have resulted in better defense approaches such as cascade adversarial training \cite{na2017cascade}, principled training \cite{certifying}. %\cite{DLres} is also based on adversarial training 

%Some researchers suggested modifying the objective function, for example, by adding stability term to encourage the network to generate similar output for images of various perturbed versions \cite{stability}, or by adding a regularization term based on adversarial perturbations to learn to defend against adversarial attacks \cite{DeepDefense}.


%Modifying the network structure was proposed as a defensive technique by, for example, adding a detector subnetwork trained to distinguish between real data and data with adversarial perturbations \cite{detector}, using a Multi-model-based defense approach (MULDEF) \cite{MULDEF} based on constructing multiple models from a target model forming a model family. The model family is designed to achieve robustness diversity by randomly choosing, at run-time, a different model to be applied to each input example.  

%These proposed defense mechanisms resulted in heavier models, requiring either additional computations or model retraining, making CNN deployment more challenging. Most of these defenses have been proven ineffective \cite{Obfuscated}, \cite{Carlini}, \cite{carlini2016evaluating} or are impractical for real-time scenarios.

%In contrast, our approach results in less computation, less power consumption and less resources without reconfiguration or loss in accuracy.

\noindent
\textbf{Randomization-based Defenses.} These techniques are the closest to our work \cite{snP2019_certif,smooth,stoch_prunning,liu2017,defense_certified}. Liu et al. \cite{liu2017} suggest to randomize the entire DNN and predict using an ensemble of multiple copies of the DNN. Lecuyer et al. \cite{snP2019_certif} also suggest to add random noise to the first layer of the DNN and estimate the output by a Monte Carlo simulation. These techniques offer a bounded theoretical guarantee of robustness. From a practical perspective, none of these works has been evaluated at scale or with realistic implementations.  For example, Raghunathan et al.~\cite{defense_certified} evaluate only a tiny neural network.  Other works~\cite{smooth,snP2019_certif} consider scalability but require high overhead to implement the defense (specifically, to estimate the model output which requires running a heavy Monte Carlo simulation involving a number of different runs of the CNN).
Our approach is different since not only our noise does not require overhead but comes naturally from the simpler and faster AC implementation. Moreover, while these techniques require additional training, DA is a drop-in replacement of the hardware without specific training requirements, and with no changes to the architecture nor the parameters of the CNN.  %In fact, the AC classifier is around 4x faster than the exact classifier, and 2.5x more energy efficient.

==> asplos21main-p898-p (Copy)/Security_evaluation.tex <==

In this section, we empirically explore the robustness properties of DA under a number of threat models.  % propose to tackle the relevance of the proposed approximation in enhancing the robustness of CNNs against adversarial attacks. 
We first explore the transferability of adversarial attacks where we evaluate whether attacks crafted for exact CNNs transfer to approximate CNNs. We then consider direct attacks against approximate CNNs in both black and white-box settings.  

%To further study the impact of approximation on CNNs robustness, we comparatively evaluate the sensitivity of approximate CNNs to input gaussian noise.

\subsection{Experimental Setup}

The first benchmark we use is the LeNet-5 CNN architecture \cite{lenet5} along with the MNIST database \cite{mnist}, which implements a classifier for handwritten digit recognition. The MNIST consists of 60,000 training and 10,000 test images with 10 classes corresponding to digits. Each digit example is represented as a gray-scale image of $28 \times 28$ pixels, where each feature corresponds to a pixel intensity normalized between 0 and 1.
We also use the AlexNet image classification CNN \cite{Alexnet} along with the CIFAR-10 database \cite{CIFAR}.  CIFAR-10 consists of 60,000 images, of dimension $64 \times 64 \times 3$ each and contains ten different classes.  LeNet-5 consists of two convolutional layers, two max-pooling layers, and two fully connected layers.  AlexNet uses five convolution layers, three max-pooling layers, and three fully connected layers. %, as shown in Table \ref{lenet5_archi} 
The rectified linear unit (ReLU) was used as the activation function in this evaluation, along with a dropout layer to prevent overfitting.
For both models, the output layer is a special activation function called softmax that will assign probabilities to each class. 
%representing a categorical distribution over class labels.


%\begin{figure}[!htp]
%\centering
%\includegraphics[width=\columnwidth]{LeNet5_architecture.pdf}
%\caption{Architecture of the LeNet-5 CNN.}
%\label{lenet5_archi}
%\end{figure}

%\begin{table}[!htp]
%\centering
%  \caption{Classifiers architectures of LeNet-5 and AlexNet.\ihsen{we may delete this table (and summarize its data in the text) since we need space}}
%  \label{lenet5_archi}
%  \begin{tabular}{cc}
%    \toprule
%     \textbf{LeNet-5}	& \textbf{AlexNet} \\
%    \midrule
%     Conv2d(1, 10, 5)            &   Conv2d(3, 32, 3)           \\
%     MaxPooling2D(2, 2)          &   ReLU()             \\
%     ReLU()                      &   Conv2d(32, 64, 3)            \\ 
%     Conv2d(10, 20, 5)           &   ReLU()            \\
%     Dropout(0.25)               &   MaxPooling2D(2, 2)   \\      
%     MaxPooling2D(2, 2)          &   Conv2d(64, 128, 3)            \\
%     ReLU()                      &   ReLU()              \\ 
%     Flatten()                   &   Conv2d(128, 128, 3)        \\ 
%     Linear(320, 50)             &   ReLU()\\
%     ReLU()                      &   MaxPooling2D(2, 2)\\
%     Dropout(0.25)               &   Dropout(0.05)   \\   
%     Linear(50, 10)              &   Conv2d(128, 256, 3)\\
%     Softmax()                   &   ReLU()\\
%                                 &   MaxPooling2D(2, 2)             \\ 
%                                 &   Dropout(0.1)  \\
%                                 &   Linear(4096, 1024)     \\
%                                 &   ReLU()  \\
%                                &   Linear(1024, 512)     \\
%                                 &   ReLU()  \\                
%                                 &   Dropout(0.1)  \\
%                                 &   Linear(512, 10)     \\
%                                 &   Softmax()    \\
%  \bottomrule
%\end{tabular}
%\end{table}

%The training parameters used to train our classifiers are presented in Table \ref{training_param}. 
Our implementations are built using the open source ML framework PyTorch \cite{PyTorch}.
We use the Adam optimization algorithm to train the LeNet-5 classifier.  For Alexnet, we use Stochastic Gradient Descent (SGD) with a learning rate equal to  $0.01$ and $0.001$, respectively.  Note that \emph{no retraining} is applied in DA, we rather use the same hyper-parameters obtained from the original (exact) classifier; we simply replace the multipliers with the approximate multiplier.

Our reference exact CNNs are conventional CNNs based on exact convolution layers with the format Conv2d provided by PyTorch.  In contrast, the approximate CNNs emulate the 32-bit Ax-FPM functionality and replace the multiplication in the convolution layers with Ax-FPM in order to assess the behavior of the approximate classifier. %This resulted in very slow simulations, which limited the test cases in terms of input size and classifier architecture. 

Since we are simulating a cross-layer (approximate) implementation from gate-level up to system-level, the experiments (forward and backward gradient) are highly time consuming, which limited our experiments to the two datasets MNIST and CIFAR-10.

%\ihsen{ $\xleftarrow[]{}$ let's keep this to the end (discussion may be)} 
Except for the black-box setting where the attacker trains his own reverse-engineered proxy/substitute model, the approximate and exact classifiers share the same pre-trained parameters and the same architecture; they differ only in the hardware implementation of the multiplier.

%\begin{table}[!htp]
%\centering
%  \caption{Training parameters of classification models.}
%  \label{training_param}
%  \begin{tabular}{ccc}
%    \toprule
%    \textbf{Parameters}& \textbf{LeNet-5}	& \textbf{AlexNet} \\
%    \midrule
%    Optimization method   & Adam    & SGD  \\
%    Learning rate         & 0.01    & 0.001\\
%    Batch Size 	          & 64      &  4\\ 
%    Epochs	              & 10      &  10\\ 
%  \bottomrule
%\end{tabular}
%\end{table}

\subsection{Do Adversarial Attacks on an Exact CNN Transfer to an Approximate CNN ?}
\label{sec:transExApx}


\textbf{Attack Scenario.} In this setting, the attacker has full knowledge of the classifier architecture and hyper-parameters, but without knowing that the model uses approximate hardware.  An example of such scenario could be in case an attacker correctly guesses the used architecture based on its widespread use for a given application (e.g., LeNet-5 in digit recognition), but is unaware of the use of DA as illustrated in Figure~\ref{grey-box}.

\begin{figure}[!htp]
\centering
\includegraphics[width=\columnwidth]{grey_box_setting1.pdf}
\caption{Transferrability attack scenario.} %\ihsen{please use "grey" or "gray" (in the figure vs text)}}
\label{grey-box}
\end{figure}

\noindent\textbf{Transferability Analysis.} The classifier generates adversarial examples using the set of algorithms in Table~\ref{Attack_methods} and assume that the exact classifier from Lenet-5 trained on the MNIST dataset. Notice that the hyperparameters, as well as the structure of the network, are the same between the exact and the approximate classifiers.  The attacker then tests the adversarial examples against the approximate classifier.  %The only difference is the underlying approximate hardware for the defender side. %We don't test the entire MNIST dataset due to time and computational constraints as emulating the multiplication to the bit level makes the testing process time consuming and computationally expensive. We choose a subset of the original dataset where different classes are randomly chosen and equivalently represented. %We use the Foolbox \cite{foolbox} tool to generate the adversarial examples.
Table \ref{grey-boxresult} presents the attacks respective success rates. We notice that the DA considerably reduces the transferability of the malicious samples and, by consequence, increases the robustness of the classifier to this attack setting. We observed that the robustness against transferability is very high, and reaches $99\%$ for $C\&W$ attack.

%Please note that this work is the first that explores the robustness properties of CNNs built using approximate circuits.

\begin{table}[!htp]
\small
  \caption{Attacks transferability success rates for MNIST.}
  \label{grey-boxresult}
  \begin{tabular}{ccc}
    \toprule
    \textbf{Attack method} & \textbf{Exact LeNet-5}  & \textbf{Approximate LeNet-5} \\
    \midrule
        FGSM          &   100\%    & 12\%    \\
        PGD           &   100\%    & 28\%    \\
        JSMA          &   100\%    & 9\%   \\
        C\&W          &   100\%    & 1\%    \\
        DF	          &   100\%    & 17\%   \\ 
        LSA	          &   100\%    & 18\%   \\ 
        BA	          &   100\%    & 17\%   \\ 
        HSJ	          &   100\%    & 2\%    \\         
  \bottomrule
\end{tabular}
\end{table}

We repeat the experiment for AlexNet with CIFAR-10 dataset. For the same setting, the success of different adversarial attacks is shown in Table \ref{attackAlexnet}.  While more examples succeed against the approximate classifier, we see that the majority of the attacks do not transfer.  Thus, DA offers built-in robustness against transferability attacks.  %We found that our proposed approach helps enhancing the resiliency of our classifier in consistency with what we proved in the theoretical study.

\begin{table}[!htp]
\small
\centering
  \caption{Attacks transferability success rates for CIFAR-10.}%\nael{No DF results?}
  \label{attackAlexnet}
  \begin{tabular}{ccc}
    \toprule
    \textbf{Attack method} & \textbf{Exact AlexNet}  & \textbf{Approximate AlexNet} \\
    \midrule

        FGSM          &   100\%    & 38\%    \\        
        PGD           &   100\%    & 31\%    \\
        JSMA          &   100\%    & 32\%   \\        
        C\&W         &    100\%  & 17\%    \\
        DF	          &   100\%    & 35\%   \\ 
        LSA	          &   100\%    & 36\%   \\ 
        BA	          &   100\%    & 37\%   \\ 
        HSJ	          &   100\%    & 12\%    \\ 
  \bottomrule
\end{tabular}
\end{table}

Notice that, unlike other state-of-the-art defenses, our defense mechanism protects the network without relying on the attack details or the model specification and without any training beyond that of the original classifier.  
Unlike most of the perturbation-based defenses that degrade the classifier’s accuracy on non-adversarial inputs, our defense strategy significantly improves the classification robustness with no baseline accuracy degradation, as we will show in Section~\ref{CNNaccuracy}.  % (this aspect is detailed in Section \ref{sec:perf_impl}.% negligible impact on non-adversarial images.%, as we showed in the previous subsection. 

%\ihsen{In the remainder of the paper, we will focus only on Ax-FPM based DA. In fact, our design outperforms HEAP-based DA in both robustness (Table \ref{grey-boxresult}) and resource utilization, while having the same overall accuracy level as shown later in Section \ref{CNNaccuracy}.} 

\subsection{Can We Attack an Approximate CNN?}

In the remaining attack models, we assume that the attacker has direct access to the approximate CNN. We consider both black-box and white-box settings.% where a powerful attacker knows the full internal details of the approximate classifier.

%----------------------------To review carefully -------------

%\subsection{Defensive approximation and adversarial samples crafting}
%This section evaluates the robustness of the approximate CNNs compared to a baseline exact implementation.  

%Similar to \cite{distillation_SP}, we define the \emph{robustness}  of a CNN to adversarial examples as its capability to resist perturbations. This could be expressed as follows: A robust CNN should (i) achieve good classification accuracy of samples both inside and outside its training dataset, as well as (ii) model a smooth classifier which is able to correctly label samples both from its training dataset and outside. 


%\ihsen{Defensive distillation has been shown week in later publications. We probably want to avoid associate our approach with it.}
%While in \cite{distillation_SP} the authors showed that distillation in a lower-size network helps the network generalize and smooths its decision boundary by reducing overfitting, AC has a similar impact without additional heavy training process.
%\ihsen{I'm not sure we want to get into the explanation here. We might let it to Section \ref{sec:how}}. 
%The primary insight is that by using AC, we are injecting noise into our calculations that modifies the decision boundary defined by the trained model. Consequently, AC results in a lower overfitting aspect thereby enhancing resilience against adversarial attacks. The AC-induced noise will be superimposed to the initial classifier and behaves as a separate input-dependent channel. As a result, AC hardware interferes with the structure of the adversarial perturbations in a way that limits the transferability from a proxy reverse-engineered model (black-box), as well as from the exact model itself (grey-box). Moreover, moving the decision boundary makes a successful adversarial example requires a higher distance from the clean sample. This makes the crafted adversarial for a white-box setting more difficult, especially when limited by the perceptibility of the adversarial example. 
%------------------------------
%------------------------------

%\ihsen{the paragraph should be starting from here I think.}\\

%To evaluate the robustness of our approximate classifier, we used a subset of the MNIST %and CIFAR-10  database correctly classified by the exact CNN as the test set. %and we use the Foolbox \cite{foolbox} tool to generate the adversarial examples%, see Figure \ref{adv}
%Notice that in this paper we only consider cases where the adversarial examples successfully fool the exact classifier.
%\begin{figure}[!htp]
%\centering
%\includegraphics[width=\columnwidth]{adversarial_examples-converti.pdf}
%\caption{Set of clean and adversarial samples for the two datasets MNIST and CIFAR-10: top row corresponds to the set of clean samples correctly classified by the exact CNN and the bottom row corresponds to the set of adversarial examples generated using LSA and misclassified by the exact CNN.}
%\label{adv}
%\end{figure}

%--------------------------------------
%--------------------------------------


%\textbf{Attack scenario:}
%\subsubsection{Black-box results}
\textbf{Black-box Attack.} In a black-box setting, the attacker has no access to the classifier architecture, parameters, and the hardware platform but can query the classifier with any input and obtain its output label.  In a typical black-box attack, the adversary uses the results of many queries to the target model to reverse engineer it.  Specifically, the adversary trains a substitute (or proxy) using the labeled inputs obtained from querying the original model (see Figure \ref{black-box}). % Notice that since the approximate and the exact classifiers have practically the same classification output labels (as we show in Section \ref{CNNaccuracy}), the substitute model is practically the same for the two models under attack. \nael{Is this an important point to make here?}
We also conduct a black box attack on the exact classifier and evaluate how successful the black box attack is in fooling it.  Essentially, we are comparing the black-box transferability of the reverse-engineered models to the original models for both the exact and the approximate CNNs. %Each adversarial example successfully transferred to the exact CNN, its transferability will be evaluated for the proposed approximate CNN.

\begin{figure}[!htp]
\centering
\includegraphics[width=\columnwidth]{black_box_setting1.pdf}
\caption{Black-box attack scenario. }
\label{black-box}
\end{figure}

In Table \ref{black-boxresult}, we present the attack success ratios for the exact CNN and the approximate/DA CNN. DA increases resilience to adversarial attacks across various attacks and for both single-step and iterative ones: it achieves $73\%$ classification success on adversarial examples in the worst case and the defense succeeded in up to $100\%$ of the examples generated by C\&W, PGD, and HSJ respectively.  %ithout re-training the classifier or any additional defense strategy. 
\begin{table}[!htp]
\small
\centering
  \caption{Black-box attacks success rates for MNIST.}
  \label{black-boxresult}
  \begin{tabular}{ccc}
    \toprule
    \textbf{Attack method} & \textbf{Exact LeNet-5}  & \textbf{Approximate LeNet-5} \\
    \midrule
        FGSM          &   100\%    & 22\%    \\
        PGD           &   100\%    & 0\%    \\
        JSMA          &   100\%    & 13\%   \\
        C\&W          &    100\%   & 0\%    \\
        DF	          &   100\%    & 25\%   \\ 
        LSA	          &   100\%    & 26\%   \\ 
        BA	          &   100\%    & 27\%   \\ 
        HSJ	          &   100\%    & 0\%    \\ 
  \bottomrule
\end{tabular}
\end{table}
%\nael{Why is the order in this table different from the order in the original attack table?}
%\subsubsection{White-box Attack }

%\subsection{White-box results}

\textbf{White-box Attack.} In this setting, the attacker has access to the approximate hardware along with the victim model architecture and parameters, as shown in Figure \ref{white-box}. In particular, the adversary has full knowledge of the defender model, its architecture, the defense mechanism, along with full access to approximate gradients used to build the gradient-based attacks. In essence, the attacker is aware of our defense, and can adapt around it with full knowledge of the model and the hardware, which is a recommended methodology for evaluating new defenses~\cite{carlini_gift}.
 

%\begin{figure*}[ht]
%\begin{subfigure}{.33\textwidth}
%  \centering
%  % include first image
%  \includegraphics[width=.8\linewidth]{loss.pdf}  
%  \caption{Loss Attack 1}
%  \label{fig:sub-first}
%\end{subfigure}
%\begin{subfigure}{.33\textwidth}
%  \centering
%  % include second image
%  \includegraphics[width=.8\linewidth]{loss2.pdf}  
%  \caption{Loss Attack 2}
%  \label{fig:sub-second}
%\end{subfigure}
%\begin{subfigure}{.33\textwidth}
%  \centering
%  % include second image
%  \includegraphics[width=.8\linewidth]{loss3.pdf}  
%  \caption{Loss Attack 3}
%  \label{fig:sub-second}
%\end{subfigure}
%\caption{Loss value while generating white-box adversarial examples for both exact and approximate CNN}
%\label{fig:fig}
%\end{figure*}

\begin{figure}[!htp]
\centering
\includegraphics[width=\columnwidth]{white_box_setting1.pdf}
\caption{White-box attack scenario.}
\label{white-box}
\end{figure}

In this scenario, we assume a powerful attacker with full access to the approximate classifier's internal model and can query it indefinitely to directly create adversarial attacks.  Although DA in production would normally reduce execution time, in our experiments, we \emph{emulate} the 32-bit Ax-FPM functionality within the approximate classifier.  As a result, this makes inference extremely slow: on average, it takes $5$ to $6$ days to craft one adversarial example on an 8th Gen Intel core i7-8750H processor with NVIDIA GeForce GTX 1050. This led us to limit the white-box experiments; we use only two of the most efficient attacks in our benchmark: $C\&W$ and DeepFool attacks, and for a limited number of examples selected randomly from our test set for different classes. 

In a white box attack, with an unconstrained noise budget, an adversary can always eventually succeed in causing an image to misclassify. Thus, robustness against this type of attack occurs through the magnitude of the adversarial noise to be added: if this magnitude is high, this may exceed the ability of the attacker to interfere, or cause the attack to be easily detectable. %in two ways: (1) The magnitude of the adversarial noise to be added: if this magnitude is high, this may exceed the ability of the attacker to interfere, or cause the attack to be easily detectable; and (2) the number of iterations, and consequently the time for producing adversarial examples: an attack that exceeds a certain limit of queries might be detected and stopped, such as the case of Cloud-based machine-learning a service platforms.   %\nael{Did we measure this second one? Could be good to see this.} \amira{No sorry we don't have this info}
%In an attempt to attack the approximate classifier in a white-box setting, we reduce the attacks benchmark  DeepFool attack. %With a high-dimensional and non-linear image space, finding the required perturbation to push the resulting image towards the decision boundary is non-trivial. 
%This attack uses a linearized approximation of the boundary to iteratively solve the problem. In each iteration, a step is made, i.e. a perturbation is added to the image, in the direction of the linearized boundary until the image crosses the original decision boundary.
%The limited number of experiments was due to, as stated previously, time and computational constraints. In this scenario, we assume a powerful attacker with full access to the approximate classifier's internal model and can query it indefinitely to directly create adversarial attacks
\begin{figure}[!htp]
\centering
\includegraphics[width=\columnwidth]{L2_DeepFool.pdf}
\caption{Required perturbations by DeepFool attack, measured using $L_2$ distance, to generate MNIST adversarial examples for approximate and exact classifiers. }
%\caption{$L_2$ values measuring distance between different clean samples from MNIST and the generated adversarial examples using DeepFool attack for approximate and exact classifiers.}
\label{L2}
\end{figure}

Figures \ref{L2} and \ref{L2_C&W}, respectively, present different measures of $L_2$ for adversarial examples crafted using DF and $C\&W$ attacking both a conventional CNN and an approximate CNN. We notice that the distance between a clean image and the adversarial example generated under DA is much larger than the distance between a clean sample and the adversarial example generated for the exact classifier. On average, a difference of $5.12$ for $L_2$-DeepFool attacks and $1.23$ for $L_2$-C\&W attack. %Herex\nael{Amira, does is it a good idea to also show the increase in L2 (e.g., saying something like "approximately doubling the L2 distance needed for the attack to succeed")}
%\nael{How much on average?  Can we help make the readers understand if this is significant?} \amira{done}  
This observation confirms that DA is more robust to adversarial perturbations since the magnitude of the adversarial noise has to be significantly higher for DF to fool DA successfully.  %This is entirely in line with our claims, as with further decision boundaries, higher perturbation magnitudes are required to change the classifier decision and by that higher distance between clean samples and malicious ones.
%We also tried to generate adversarial examples using C\&W attack $L_2$ . The limited number of examples is due to the time required to run this attack, 
%Figure \ref{L2_C&W} shows the $L_2$ metric for adversarial examples generated by C\&W where a similar advantage holds for DA.  C\&W can generate attacks with lower L2 than DF.  %for adversarial examples generated using $C\&W$ comparatively between an exact and an approximate CNN. The same observation is made: higher perturbation is required to push an input image across the decision boundary of an approximate model. 

To understand the implication of this higher robustness in terms of observable effects on the input image,  we also show the Peak Signal to Noise Ratio (PSNR) and the Mean Square Error (MSE) in Figures \ref{MSE&PSNR_DF} and \ref{MSE&PSNR}; these are two common measures of the error introduced in a reconstruction of an image. Specifically,  MSE represents the average of the squares of the "errors" between the clean image and the adversarial image. The error is the amount by which the values of the original image differ from the distorted image. PSNR is an expression for the ratio between the maximum possible value (power) of a signal and the power of distorting noise that affects the quality of its representation. It is given by the following equation: $P S N R=20 \log _{10}\left(\frac{M A X_{x}}{\sqrt{M S E}}\right)$. The lower the PSNR, the higher the image quality degradation is.

We notice that the adversarial examples generated for DA is more noisy than adversarial examples generated for an exact classifier. The PSNR difference reaches $4 dB$ for C\&W and $7.8dB$ for DeepFool. Moreover, on average, the DA-dedicated adversarial examples have $6$ times, and $3$ times more MSE than the exact classifier-dedicated adversarial examples for $C\&W$ and DeepFool attacks, respectively. 
%Deepfool:Appx: 0.12Exact: 0.02
%C&W:Appx: 0.015 Exact: 0.005

% than the ones generated using exact model and are no longer imperceptible. 

\begin{figure}[!htp]
\centering
\includegraphics[width=0.9\columnwidth]{L2_C_W.pdf}
\caption{Required perturbations by C\&W attack, measured using $L_2$ distance, to generate MNIST adversarial examples for approximate and exact classifiers. }
%\caption{$L_2$ values measuring distance between different clean samples from MNIST and the generated adversarial examples using C\&W attack for approximate and exact classifiers.}
\label{L2_C&W}
\end{figure}

We can conclude that DA provides substantial built-in robustness for all three attack models we considered.  Attacks generated against an exact model do not transfer successfully to DA.  Black-box attacks also achieve a low success rate against DA.  Finally, even white-box attacks require substantial increases in the injected noise to fool DA.  Next, we probe deeper into DA's internal behavior to provide some intuition and explanation for these observed robustness advantages.% proposed approximation made the classifier not only more robust against transferability but also harder to use to create imperceptible malicious samples. These observations confirm the impact of AC-induced noise towards enhancing the generalization of the classifier. 

\begin{figure}[!htp]
\centering
\includegraphics[width=\columnwidth]{MSE_PSNR_DF.png}
\caption{MSE and PSNR values for the generated adversarial examples using DeepFool method when attacking the approximate and the exact classifiers.}
\label{MSE&PSNR_DF}
\end{figure}

\begin{figure}[!htp]
\centering
\includegraphics[width=\columnwidth]{MSE_PSNR.png}
\caption{MSE and PSNR values for the generated adversarial examples using $L_2$-C\&W method when attacking the approximate and the exact classifiers.}
\label{MSE&PSNR}
\end{figure}






%\subsection{How does approximate computing help CNNs security?}





==> asplos21main-p898-p (Copy)/Threat_model.tex <==
We assume an attacker attempting to conduct adversarial attacks to fool a classifier in a variety of attack scenarios.%, which we overview in this section.  

\subsection{Adversary Knowledge (Attacks Scenarios)}

In this work, we consider three attack scenarios:

\noindent
    \textbf{\textit{Transferability Attack.}} We assume the adversary is aware of the exact classifier internal model; its architecture and parameters. The adversary uses the exact classifier to create adversarial examples. Thus, we explore whether these examples transfer effectively to the approximate classifier (DA classifier).
    
  \noindent  
    \textbf{\textit{Black-box Attack.}} We assume the attacker has access only to the input/output of the victim classifier (which is our approximate classifier) and has no information about its internal architecture.  The adversary first uses the results of querying the victim to reverse engineer the classifier and create a substitute %\khaled{proxy or substitute?} 
    CNN model.   With the substitute model, the attacker can attempt to generate different adversarial examples to attack the victim classifier.

\noindent
    \textbf{\textit{White-box Attack.}} We assume a powerful attacker who has full knowledge of the victim classifier's architecture and parameters (including the fact that it uses AC).  The attacker uses this knowledge to create adversarial examples.  % and the defense strategy used which means that the adversary is capable of generating adversarial examples targeting the victim classifier.  


\subsection{Adversarial Example Generation}

 We consider several adversarial attack generation algorithms for our attack scenarios, including some of the most recent and potent evasion attacks.  Generally, in each algorithm, the attacker tries to evade the system by adjusting malicious samples during the inference phase, assuming no influence over the training data. However, as different defenses have started to be deployed that specifically target individual adversarial attack generation strategies, new algorithms have started to be deployed that bypass these defenses. For example, methods such as defensive distillation \cite{distillation_SP} and automation detection \cite{early} were introduced and demonstrate robustness against the Fast gradient sign attack %\khaled{what is this attack?}
 \cite{fgsm}.  However, the new $C\&W$ attack was able to bypass these defenses \cite{CW}.  
Thus, demonstrating robustness against a range of these attacks provides confidence that a defense is effective in general, against all known attack strategies, rather than against a specific strategy.

These attacks can be divided into three categories: Gradient-based attacks relying on detailed model information, including the gradient of the loss w.r.t. the input. Score-based attacks rely on the predicted scores, such as class probabilities or \textit{logits} of the model. On a conceptual level, these attacks use the predictions to estimate the gradient numerically.  Finally, decision-based attacks rely only on the final output of the model and minimizing the adversarial examples' norm.  The attacks are summarized in Table \ref{Attack_methods}. %\textcolor{red}{Khaled: it is not clear to me what does "and minimizing the norm-based adversarial examples" mean} % and described in more detail in the order they appear in the table below. %In the following we describe each attack in more detail. % used to generate adversarial examples. %\ihsen{We might want to include the previous attacks too, since we already have their results.}


\begin{table}[!htp]
\small
\centering
  \caption{Summary of the used attack methods. Notice that the strength estimation is based on~\cite{strength}.} 
  \label{Attack_methods}
  \begin{tabular}{ccccc}
    \toprule
    \textbf{Method} & \textbf{Category}  & \textbf{Norm} & \textbf{Learning} & \textbf{Strength} \\
    \midrule
    FGSM~\cite{fgsm}  & gradient-based   &  $L_\infty$  & One shot  & ***\\
    PGD~\cite{pgd}   & gradient-based   &  $L_\infty$  & Iterative & ****\\
    JSMA~\cite{SMA}  & gradient-based   &  $L_0$       & Iterative & ***\\
    C\&W~\cite{CW}  & gradient-based   &  $L_2$       & Iterative & *****\\
    DF~\cite{deepfool}    & gradient-based   &  $L_2$       & Iterative & ****\\
    LSA~\cite{localsearch}   & Score-based      &  $L_2$       & Iterative & ***\\
    BA~\cite{BA}    & Decision-based   &  $L_2$       & Iterative & ***\\
    HSJ~\cite{HSJ}    & Decision-based   &  $L_2$       & Iterative & *****\\
%    Universal perturbations & & Untargeted & Universal & $L_2$ & Iterative & *****\\
    
  \bottomrule
\end{tabular}
\end{table}


% \nael{Would be nice if we can provide some insights about the strengths and weaknesses of the attacks rather than just describing what they do mechanically.  Some descriptions are really unclear both in terms of how they work and the implications of the strategy (e.g., BA).  Others, such as DF are described very nicely. }


% \noindent \textbf{Fast Gradient Sign Method (FGSM).} The Fast Gradient Sign Method \cite{fgsm} is a single-step, gradient-based, attack. An adversarial example is generated by performing a one step gradient update along the direction of the sign of gradient at each pixel as follows:

%  \begin{equation}
%      x^* = x + \epsilon \cdot sign (\nabla_{x}\mathcal{L}_{\theta}(x,y))
%  \end{equation}
% Where $\nabla \mathcal{L}()$ computes the gradient of the loss function $\mathcal{L}$ and $\theta$ is the set of model parameters. The $sign()$ denotes the sign function and $\epsilon$ is the perturbation magnitude. 

% \noindent \textbf{Projected gradient descent (PGD).} PGD \cite{pgd} is a the strongest iterative variant of the FGSM where the adversarial example is generated as follows:
%  \begin{equation}
% x^{t+1} = \mathcal{P}_{\mathcal{S}_x}(x^t + \alpha \cdot sign (\nabla_{x}\mathcal{L}_{\theta}(x^t,y)) )
%  \end{equation}
% Where $\mathcal{P}_{\mathcal{S}_x}()$ is a projection operator projecting the input into the feasible region $\mathcal{S}_x$ and $\alpha$ is the added noise at each iteration.
% The PGD attack tries to find the perturbation that maximizes the loss of a model on a particular input while keeping the size of the perturbation smaller than a specified amount. %\nael{What is alpha?  ARe the rest of the parameters the same as FGSM?} \khaled{maybe we should just mention here that alpha is the same as epsilon in FGSM}


% \noindent \textbf{Jacobian based saliency map attack (JSMA).} Jacobian based saliency map attack \cite{SMA} builds a saliency map using the Jacobian matrix in order to define the most salient input pixels to be modified. The Jacobian matrix of a given input $x$ is computed as follows: 
% \begin{equation}
%     J_{F}(x) = \frac{ \partial F(x)}{ \partial x} =  \left[\frac{ \partial F_{j}(x)}{ \partial x_{i}}\right]_{i \times j}
% \end{equation}
% Where $F$ denotes the second-to-last layer in \cite{SMA}. 


% \noindent \textbf{Carlini \& Wagner (C\&W).} The Carlini \& Wagner attack (C\&W) \cite{C&W} is one of the state-of-the-art attacks. This latter has 3 forms based on different distortion measures ($l_0, l_2, l_{\infty}$). In this work we only consider the $l_2$ form as it has the best performance. It generates adversarial examples by solving the following optimization problem:

%  \begin{equation}
%      \begin{array}{rrclcl}
%         \displaystyle \minimize_{\delta} & \multicolumn{3}{l}{\left\Vert \delta \right\Vert_2 + c\cdot l(x+\delta)}\\
%         \textrm{s.t.} & x + \delta \in [0,1]^n 
% \end{array}
%  \end{equation}
% Where $\left \Vert \delta \right \Vert_2$ is the smallest perturbation measured by the $l_2$ norm that makes the model missclassify into another/target class. $l(\cdot)$ is the loss function reflecting the distance between the current situation and the objective of the attack defined as:

%  \begin{equation}
% l(x) = max(max_{i \neq t } \{Z(x)_i\}-Z(x)_t - \kappa )
%  \end{equation}
 
% Where $Z(x)$ is the output of the layer before the softmax called \textit{logits}. $t$ is the target label, and $\kappa$ is called the confidence, a hyper-parameter used to enhance the transferability of the output. 
% An adversarial example is considered as successful if $max_{i \neq t}\{Z(x)_i\}-Z(x)_t \leq 0$. In the C\& W attack, the box constrained optimization problem $x + \delta \in [0,1]^n$ is turned to an unconstrained problem by replacing $\delta$ with $\frac{1}{2}(tanh(w)+1)-x$, where$w$ is a new optimizer ranging in $(-\infty , +\infty)$.

% \noindent \textbf{DeepFool Attack (DF).} DeepFool attack \cite{deepfool} is an iterative attack optimized for the $L_2$ metric where the basic idea is to find the closest decision boundary from a clean image $x$ in the image space, and then to go beyond that boundary to fool the classifier. It is hard to solve this problem directly in the high-dimensional and highly non-linear space in neural networks. So instead, it iteratively solves this problem with a linearized approximation. Specifically, for each iteration, it linearizes the classifier around the intermediate $x^*$ and derives an optimal update direction on this linearized model. It then updates $x^*$ towards this direction by a small step $\alpha$. By repeating the linearize-update process until $x^*$ crosses the decision boundary, the attack finds an adversarial example with small perturbation. 

% \noindent \textbf{Local Search Attack (LSA).} Local Search Attack \cite{localsearch} is an iterative attack that utilizes a local-search based technique to construct a numerical approximation to the network gradient, which is then carefully used to construct a small set of pixels in an image to perturb. This attack only uses the prediction results of the target model and does not require gradients nor probabilities. 

% \noindent \textbf{Boundary Attack (BA).} Boundary Attack \cite{BA} is an iterative algorithm based on rejective sampling algorithm in combination with a simple proposal distribution. Starting from a large perturbation sampled at each step from the proposal distribution, reducing the distance between the perturbed image and the original input. In addition to its simplicity, this attack is extremely flexible in terms of the possible adversarial criteria and has a performance similar to that of gradient-based attacks in terms of the size of minimal perturbations.


% \noindent \textbf{Hop Skip Jump Attack (HSJ).} HSJ \cite{HSJ} is a powerful black-box attack that only requires final class predictions. This method builds an approximate gradient and estimates the gradient direction using binary information at the decision boundary.


==> asplos21main-p898-p (Copy)/how.tex <==
In this section, we probe into the DA classifier's operation to attempt to explain the robustness advantages we observed empirically in the previous section.  %Given the promising empirical results shown in the previous section, we attempt in this section to provide an analysis of the defensive approximation mechanism. %the eventual mechanisms that are involved in the security enhancement due to approximate computing. 
While the explainability of deep neural networks models is a known hard problem, especially under adversarial settings~\cite{samek2019explainable}, we attempt to provide an overview of the mechanisms that we think are behind the DA impact on security. %Before proceeding further, notice that our purpose in this section is not to provide a definitive argument about the explanation of the AC impact on robustness, but rather we view it as an initial step towards drawing an explanation that connects the circuit-level approximation to the model robustness for future work to build upon.  
We study the impact of the approximation on CNNs' confidence and generalization property. We follow this analysis in the Appendix with a mathematical argument explaining the observed robustness based on recent formulations by Lecuyer et al.~\cite{snP2019_certif}. %we analyze the approximate computing impact on the gradient, which is a key player in adversarial attacks generation process, and we provide a theoretical basis inspired from \cite{snP2019_certif}.

%\subsection{Impact of approximation on model confidence}
%\label{subsec:confidence}
%\noindent \textit{Impact of approximation on model confidence}\\
%\ihsen{The confidence study might move to later in the paper. }

The output of the CNN is computed using the \emph{softmax} function, which normalizes the outputs from the fully connected layer into a likelihood value for each output class.  Specifically, this function takes an input vector and returns a non-negative probability distribution vector of the same dimension corresponding to the output classes.   In this section, we examine the impact of approximation on the observed classifier confidence. We compare the output scores of an exact and an approximate classifier for a set of $1000$ representative samples selected from the MNIST dataset: $100$ randomly selected from each class. We define the classification confidence, $C$, as the difference between the true class $l$'s score and the "runner-up" class score, i.e., the class with the second-highest score. $C$ is expressed by $C = output[l] - max_{j \neq l} \{output[j]\}$.  The confidence ranges from $0$ when the classifier gives equal likelihood to the top two or more classes, to $1$ when the top class has a likelihood of $1$, and all other classes $0$.  


%\begin{equation}
%\label{eq:confidence}
%    C = output[l] - max_{j \neq l} \{output[j]\}
%\end{equation}

%Figure \ref{difference} shows a scatter-plot representation of the confidence of both classifiers for the 1000 image sample set.  On each point on the x-axis, we plot the confidence of that the DA classifier and the exact classifier for a particular image.  It is clear the confidence of the approximate classifier is substantially higher, clustering near 1.   In fact, for  $97.6\%$ of the images, DA has increased the confidence in the true class compared to other classes.  

We plot the cumulative distribution of confidence for both classifiers in Figure \ref{conf_dis}.  DA images have higher confidence; for example, in images classified by the exact classifier, less than $20\%$  had higher than $0.8$ confidence.   
On the other hand, for the approximate classifier, $74.5\%$ of the images reached that threshold.



%\begin{figure}[!htp]
%\centering
%\includegraphics[width=\columnwidth]{confidence.pdf}
%\caption{Difference in confidence of exact and approximate model for clean image samples from  MNIST.}
%\label{difference}
%\end{figure}

\begin{figure}[!htp]
\centering
\includegraphics[width=0.9\columnwidth]{confidence_dist.pdf}
\caption{Cumulative distribution of confidence.}
\label{conf_dis}
\end{figure}



%\begin{figure}[!htp]
%\centering
%\includegraphics[width=\columnwidth]{confidence_dist2.pdf}
%\caption{Percentage of input images and its corresponding confidence.}
%\label{conf_dis}
%\end{figure}
Compared to the baseline feature maps generated from an exact convolution operation, for the same pre-trained weights, our approximate convolution highlights further the features. Recall that the multiplier injected noise is higher when input numbers are higher (i.e., there is a high similarity between the kernel and the input data) and lower when the inputs are lower (when the similarity is small), as shown in Figure \ref{appx_conv}. We believe that these enhanced features continue to propagate through the model resulting in a higher probability for the predicted class. This higher confidence requires thereby higher noise to decrease the true label's likelihood, and increase another label's.  %This aspect can be theoretically modeled as detailed in the Appendix.

%HEREx\nael{Can we connect confidence to robustness as we do now in the intro?  A sentence or two are fine}
%\subsection{ Impact of approximation on gradient}
%\noindent \textit{Impact of approximation on gradient}\\
%When crafting adversarial examples using gradient-based attacks, a similar concept to that used in back-propagation, one of the most used training algorithm, is usually used by considering the model parameters to be constant and the inputs to be variable and computing the gradients corresponding to each input. These gradients are used to obtain the perturbation vector that turns a clean input image to a malicious input missclassified by the same model. 

%Obfuscated gradient can give a false sense of security it is considered as a special case of gradient masking, when following the gradient does not increase optimize the loss and does not lead to a successful attack

%Now considering the proposed approximate model, the forward pass, as previously stated, is computed by replacing the exact convolution operation between the input images and the exact model pretrained hyper-parameters in $y = w * x + b$ with an approximate convolution $y = w \circledast x + b$. When computing back-propagation, the backward pass of an approximate convolution layer is calculated by replacing the exact multiplication with the proposed approximate multiplication. For instance, the approximate output gradient and the approximate input gradient %, weight gradient, and bias gradient are respectively computed as follows:
%\begin{align}
%   dy & = \frac{\delta L}{\delta y} \\
%   dx &= \frac{\delta L}{\delta x} =  \frac{\delta L}{\delta y} \circledast \frac{\delta y}{\delta x}  = dy \circledast w
%\end{align}

%Where $*$ refers to the exact convolution, $\circledast$ refers to the approximate convolution, $x$ refers to the input data, $w$ refers to the weights, $b$ refers to the biases, and $L$ refers to the loss function.

%Unlike other defenses that cause Shattered Gradients whether intentionally or unintentionally, by using non-differentiable operations, introducing numeric instability, or causing a gradient to be nonexistent or incorrect \cite{Obfuscated}, our defense maintain differentiable operations: the gradient calculation method is the same as for an exact model only replacing the exact multiplication with an approximate multiplication. As shown in Figure \ref{fig:sub-first}, plotting the loss function when generating an adversarial example using the PGD attack, we can see that the gradient is globally maximizing the classification loss, the small fluctuations are due to the discontinuity of the noise introduced by the approximate multiplier.
%Unlike randomized defenses, where either the network itself is randomized or the input is randomly transformed before being fed to the classifier, our method does not cause Stochastic Gradients. As even though we are approximating the multiplication result our calculations remain deterministic.


%\begin{figure}[ht]
% \centering
%  % include first image
% \includegraphics[width=\linewidth]{Loss_function.pdf}  
% \caption{Loss when crafting AE using PGD Attack. }%(unsuccessful attack for both models)}
% \label{fig:sub-first}
%\end{figure}
%For an exact model, the exact output gradient, the exact input gradient, the exact weights gradient, and the exact bias gradient are respectively computed as follows: 
%\begin{align}
%   dy &= \frac{\delta L}{\delta y} \\
%   dx &= \frac{\delta L}{\delta x} =  \frac{\delta L}{\delta y} * \frac{\delta y}{\delta x}  = dy * w \\
%   dw & = \frac{\delta L}{\delta y} * \frac{\delta y}{\delta w} = dy * \frac{\delta y}{\delta w}\\
%   db &= \frac{\delta L}{\delta y} = dy * \frac{\delta y}{\delta b} 
%\end{align}

% \begin{figure}[ht]

%Our defense does not lead to Exploding/Vanishing Gradients that are often caused by defenses that consist of multiple iterations of neural network evaluation, feeding the output of one computation as the input of the next which is not our case.

%  \centering
% %  % include first image
%  \includegraphics[width=\linewidth]{loss2.png}  
%  \caption{Loss when crafting AE using PGD Attack (successful attack for both models) }
%  \label{fig:sub-first}
% \end{figure}
%----------------------------------
%\subsection{Theoretical Analysis}  %HEREx\nael{Need to come up with a better title for this section}
%----------------------------------
% We now explore the impact of approximation on the classifier robustness leveraging some formulations from Differential Privacy (DP)~\cite{diff_priv}. %Before proceeding further, note that our purpose in this subsection is not to provide a definitive argument about using approximate computing to defend against adversarial attacks, but rather we view it as an initial step towards drawing an explanation that connects the circuit-level approximation to the model robustness for future work to build upon. 
% %Specifically, while the explainability of deep neural networks behavior is a challenging task, especially under adversarial settings, we attempt to provide an overview on the mechanisms that we think are behind the defensive approximation impact on security. 
% %\ihsen{Attempt starts here}\\
% Our formulation is based on recent similar formulations for certified robustness analysis~\cite{smooth,snP2019_certif}. These prior works studied the impact of randomization on robustness by adding random Gaussian noise to all layers of a CNN.%HEREx\nael{Random is imprecise -- is Gaussian accurate?  If not, what distributions of noise did they consider?} 
% While the noise injected by DA follows a different distribution and is input dependent rather than stochastic, we believe that the theoretical analysis provides insights into the possible mechanisms that improve the robustness of DA.
% %is a theoretical analogy with our work that we develop in the following.   

% In this analysis, we formally model the problem as follows:
% Let $x$ be an input sample and $h$ a conventional classifier. We denote $\hat{h}(x) = h(x) + \triangle(x)$ the defender implementation where $\triangle(x)$ is the data dependent randomness added by the approximate circuit. In this analysis, we use the concept of Differential Privacy (DP) \cite{diff_priv}, \cite{DP}, which is concerned whether the output of a computation over a given database can reveal information about individual records in the database. %In the context of insuring data privacy, these papers suggest injecting a level of randomness 
% To prevent such data leakage, randomness is introduced in the computation, and DP is accordingly defined as follows: 

% \begin{definition} 
%     A randomized algorithm $A$ that takes as input a database $d$ and outputs a value in a space $O$ is said to satisfy ($\varepsilon$, $\delta$)-DP w.r.t. a metric $\rho$ if, for any databases $d$ and $d^{\prime}$ with $\rho(d,d^{\prime}) \leqslant1$, and for any subset of possible outputs $S \subseteq O$, we have:
%     \begin{equation}
%         P(A(d) \in S) \leq e^{\varepsilon} P\left(A\left(d^{\prime}\right) \in S\right)+\delta
%     \end{equation}
% \end{definition}

% Out of this definition, Expected Output Stability Bound, a key property of DP is deduced; the expected value of an ($\varepsilon$, $\delta$)-DP algorithm with bounded output is not sensitive to small changes in the input.
% %\ihsen{next lemma needs more introduction, to match randomization to approximation. A small figure would be perfect. UPDATE: actually we do not need to bring this Lemma here. Go directly to corollary! UPDATE: Nope, the rest of the logic doesn't make sense. Keep it -for now-}


% % \begin{lemma}
% % \label{lemma1}
% % Suppose a randomized function $A$, with bounded output $A(x) \in [0, b], b \in \mathbb{R}^{+}$, satisfies $(\varepsilon, \delta)$-DP. Then the expected output meets the following property: 
% % \begin{center}
% %     $\forall \alpha \in B_{p}(1) . \mathbb{E}(A(x)) \leq e^{\epsilon} \mathbb{E}(A(x+\alpha))+b \delta$
% % \end{center}
% % \end{lemma}

% The intuition behind using the analogy with DP in the context of robustness to adversarial examples is to create an approximate classifier such that, given an input example, the predictions are DP with regards to the features of the input (e.g., the pixels of an image). In this setting, we can derive stability bounds for the expected output of the randomized classifier, i.e., the approximate classifier. The bounds can be interpreted as a certification for robustness to adversarial examples. In our method, the added approximate noise $\triangle(x)$ for a given input $x$ has a similar effect to randomization.


% Formally, to frame the DP into our setting, regard the feature values (e.g., pixels) of an input $x$ as the records in a database.  Let $B_{p}(r):=\left\{\alpha \in \mathbb{R}^{n}:\|\alpha\|_{p} \leq r\right\}$ be the $p$-norm ball of radius $r$. For a given classification model, $h$, and a fixed input, $x \in \mathbb{R}
% ^n$, an attacker is able to craft a successful adversarial example of size $L$ for a given $p$-norm if they find $\alpha \in  B_{p}(L)$ such that $h(x + \alpha) \neq h(x)$. Now, consider an approximate classifier $\hat{h}$ that, on input $x$, outputs scores $\left(y_{1}(x), \ldots, y_{K}(x)\right) \text { (with } y_{k}(x) \in[0,1]$ and $\sum_{k=1}^{K} y_{k}(x)=1)$. 


% Combining Lemma $1$ and Corollary $1$ in \cite{snP2019_certif} directly implies bounds on the expected output on an approximate classifier:
% \begin{theorem}
% Suppose an approximate function $\hat{h}$ satisfies $(\varepsilon, \delta)$-DP w.r.t. a $p$-norm metric, and where $\hat{h}(x)=\left(y_{1}(x), \ldots, y_{K}(x)\right), y_{k}(x) \in[0,1]$:
% \begin{equation}
% \label{eq:dp}
%     \forall k, \forall \alpha \in B_{p}(1) . \hat{h}_{k}(x) \leq e^{\varepsilon} \hat{h}_{k}(x+\alpha) +\delta.%~ \footnote{This corollary and the detailed proofs can be found in \cite{snP2019_certif}} 
% \end{equation}
% \end{theorem}

% Now, consider $\alpha \in B_p(1)$, and let $x^* = x + \alpha$. From Equation \ref{eq:dp}, we have: \textbf{(i)} $\hat{h}_{k}(x) \leqslant e^\varepsilon \hat{h}_{k}(x^*) + \delta$, and
% \textbf{(ii)} $\hat{h}_{i\neq k}(x^*) \leqslant e^\varepsilon \hat{h}_{i\neq k}(x) + \delta$.

% Practically, \textbf{(i)} gives a lower-bound on $\hat{h}_{k}(x^*)$ and \textbf{(ii)} gives an upper-bound on  $\hat{h}_{i\neq k}(x^*)$.

% These elements confirm a theoretically verifiable bounded impact of an adversarial perturbation in the input on the approximate classifier's output. 


% To further investigate the robustness guarantee, suppose that when the base classifier $h$ classifies an input $x$ the most probable class $k$ is returned with probability $p_k$, and the “runner-up” class is returned with probability $p_{i\neq k}< p_k$. Based on \cite{smooth}, our approximate classifier is robust around $x$ within the $\ell_{2} \text { radius } R=\frac{\sigma}{2}\left(\Phi^{-1}\left(p_{k}\right)-\Phi^{-1}\left(p_{i}\right)\right)$, where $\Phi^{-1}$ is the inverse of the standard Gaussian CDF. This result also holds if we replace $p_k$ with a lower bound $\underline{{p}_{k}}$  and we replace $p_i$ with an upper bound $\overline{p_{B}}$. Hence, based on Theorem 1 in \cite{smooth}:

% \begin{theorem}
% \label{theorem:smooth}
% Let  $h: \mathbb{R}^{d} \rightarrow \mathcal{Y}$ be any baseline classifier, and let $\varepsilon \sim \mathcal{N}\left(0, \sigma^{2} I\right)$. Let $\hat{h}$ be the approximate implementation of $h$. Suppose $c_{k} \in \mathcal{Y} \text { and } \underline{p_{k}}, \overline{p_{i}} \in[0,1]$ satisfy:

% \begin{equation}
%     \mathbb{P}\left(h(x+\varepsilon)=c_{k}\right) \geq \underline{p}_{k} \geq \overline{p_{i}} \geq \max _{c \neq c_{k}} \mathbb{P}(h(x+\varepsilon)=c)
% \end{equation}

% Then $\hat{h}(x+ \delta) = c_k$ for all $\|\delta\|_{2}<R$, where 
% \begin{equation}
% \label{eq:theorem_smooth}
%     R=\frac{\sigma}{2}\left(\Phi^{-1}\left(\underline{p_{k}}\right)-\Phi^{-1}(\overline{p_{i}})\right)
% \end{equation}

% \end{theorem}

% Notice that Theorem \ref{theorem:smooth} insures a certified radius $R$ that is large when: (1) the noise level $\sigma$ is high, (2) the probability of the top class $c_k$ is high, and (3) the probability of each other class $c_{i \neq k}$ is low.

% Conditions (2) and (3) of high radius basically mean a higher confidence in the sense of Equation \ref{eq:confidence}. This is coherent with the results obtained in terms of robustness, given Figure \ref{conf_dis}.

% The randomization technique proposed in \cite{snP2019_certif} and \cite{smooth} uses a totally random noise that is uncorrelated to the input. This led them to use heavy Monte Carlo simulations to estimate the randomized classifier's output, which induces a considerable time overhead limiting the applicability of these techniques, especially in time critical applications. In our approach, the noise is injected at circuit-level through the approximate design and is not artificially generated from an outside source. Moreover, the correlation to the input that highlights useful features in the convolution output gives higher confidence and thereby ensures a higher robustness radius in the sense of Theorem \ref{theorem:smooth}.


% % \ihsen{----------------------------\\ Attempt ends here\\         ----------------------------}



% % This analysis is split in two folds depending on the threat model:  \\

% % \textbf{(i) White-box Setting:}
% % Consider an attacker that has full access to the defender classifier implementation $\hat{h}$. Starting from a sample inout $xB$, and based on the gradient (direction or sign), the attacker maximizes the loss of the victim classifier by adding adversarial noise $\alpha$ in the purpose of crossing the decision boundary. Under unlimited noise budget, this attack would work on any classifier. However, we want to give an intuition why defensive approximation makes white-box attacks harder to implement and needs higher noise magnitude.

% % \ihsen{Based on the distance to the decision boundary that is higher in the Approximate case $\Rightarrow$ higher noise necessary to generate an adversarial example}



% % \textbf{(ii) Transferability:} Now, we focus on the transferability of adversarial examples generated for an exact classifier to an approximate classifier.
% % For the sake of simplification, we consider a two-class problem ( $l$ and $l^*$ ). Let $H$ be the class of possible classifiers a learning system considers. Let $P$ be the probability distribution over data instances (x,y), where x is an input vector, and y is a label in $\{l,l^*\}$. Let $h \in H$ be an exact classifier to which the attacker has full access. 
% % Let $Z^l(x)$ refer to the $l$-class weight, that $h$ internally uses to classify an input $x$.
% % In a 2D space, we geometrically model $Z^l(x)$ as the distance between $x$ and the decision boundary of a classier $h$, hereby denoted $B_h ~ s.t. ~ Z^l(x) = |d^l(x, B_h)| $, where $d^l \in \mathbb{Z}$ is a scalar distance that is positive if $h(x) = l$, and negative elsewhere: 
% % \begin{equation}
% %     \left\{\begin{array}{c}
% %  if \quad d^l(x, B_h)(x) > 0, h(x)=l \\
% % if \quad  d^l(x, B_h) \leqslant 0, h(x)=l^{*}
% % \end{array}\right.
% % \end{equation}

% % We refer to as \emph{noise} and note $\delta$, the perturbation added by the attacker to an input $x$ to change its classification using $h$, and for simplicity we represent it geometrically as a one dimensional noise (it can be seen as a projection of a 2D noise) as illustrated in Figure \ref{fig:theory1}.

% % \begin{figure}[ht]
% %  \centering
% %  \includegraphics[width=\linewidth]{theory1.pdf}  
% %  \caption{Illustration of the problem in 2D, 2-class}
% %  \label{fig:theory1}
% % \end{figure}

% % As defined in \cite{confidenceICLR}, we denote $\kappa \geqslant 0$ a value that represents the attack confidence margin. Notice that  $\kappa$ is generally arbitrarily small due to Equation \ref{eq:adv}. 

% % Let be $x^* = x + \delta$ an adversarial example generated by the attacker targeting $h ~s.t. ~ h(x+\delta) = l^*$. Hence:
% % \begin{equation}
% % \label{kappa}
% %      d^l(x+ \delta, B_h) = - \kappa, \textit{and }\\
% %      Z^{l^*}(x+\delta) = \kappa
% % \end{equation}


% % Consider $\hat{h} \in H$ a learning system that corresponds to the defender implementation of an approximate classifier such that  $\hat{Z}^l(x) = Z(x) + \triangle(x)$, where $\triangle$ represents the impact of the approximation on the initial exact classifier. We assume that $\triangle(x) \geqslant 0$ based on the interpretation of the confidence results in Section \ref{subsec:confidence} which show a higher confidence afforded by the approximate model in more than $97\%$ of the cases.

% % Studying the transferability of $x^*$ can be done by verifying the sign of $d^l(x+ \varepsilon, B_{\hat{h}})$, where $B_{\hat{h}}$  represents the decision boundary of the approximate classifier. Hence,
% % \begin{equation}
% %     \hat{Z}^l(x+ \varepsilon) = Z(x + \varepsilon) + \triangle(x + \varepsilon)
% % \end{equation}


% % Given Equation \ref{kappa}, we have: 
% % \begin{equation}
% %     \hat{Z}^l(x+ \varepsilon) = |\triangle(x + \varepsilon) - \kappa|
% % \end{equation}

% % and:
% % \begin{equation}
% % \label{eq:transf}
% %       d^l(x+ \varepsilon, B_{\hat{h}}) = \triangle(x + \varepsilon) - \kappa
% % \end{equation}


% % \ihsen{NB: while $\varepsilon$ is crafted such that it affects $h()$, notice that $\triangle()$ is $\varepsilon$-agnostic }

% % Equation \ref{eq:transf} reveals two observations: First, it shows the possible transferability of adversarial examples from exact to approximate implementation as far as  $\triangle(x + \varepsilon) - \kappa \leqslant 0$. This has been observed in Section \ref{sec:transExApx} in Tables \ref{grey-boxresult} and \ref{attackAlexnet}. The second observation is that the more sneaky and effective (from the attacker perspective) the attack is, the less likely to transfer to the approximate classifier. In fact, while $\kappa$ is arbitrarily small, the smaller it is the less perceptible the distortion. On the other hand, the smaller $\kappa$, the more likely $\triangle(x + \varepsilon) - \kappa$ to be positive, and consequently the more likely the attack not to transfer.   


% % %\textbf{(ii) Reverse Engineering (Black-box):}
% % %Now consider an attacker that designs a reverse-engineered learning system. This latter  repeatedly queries the defender classifier to learn its behavior and transfer adversarial attacks to it. 

% % % \ihsen{\begin{itemize}
% % %     \item Learnability theory $\Rightarrow$ possibility of reverse engineering with arbitrarily small error.
% % %     \item gradient analysis that impacts the generated adversarial examples
% % % \end{itemize}}


% % % From the previous subsection, if a clean input sample $x$ such that $f(x)= l$, we have:
% % % \begin{equation}
% % % \label{eq:basis}
% % %   \exists \gamma /  P [d\left(x, B_{f^*}^{l}\right) \geqslant d\left(x, B_{f}^{l}\right) ] \geqslant 1 - \gamma
% % % \end{equation}
% % % Where $B_{f}$ and $B_{f^*}$ represent the decision boundary of the classifiers $f$ and $f^*$ respectively. 

% % % To prove that the approximate classifier $f^*$ is more robust to adversarial attacks than $f$, we propose first to show that:\\
% % % (i) An adversarial example crafted for $f$ is not likely transferable to $f^*$ and\\
% % % (ii) An adversarial example crafted for $f^*$ is likely transferable to $f$.

% % % Let be $\hat{x} = x + \delta$ an adversarial example crafted for a classifier $f$ such that $f(x)= l$ and $f(x+\delta)= l^*$. To prove (i), we suggest to prove Equation \ref{eq:proof(i)}.
% % % \begin{equation}
% % % \label{eq:proof(i)}
% % %     \exists \eta \in [0, \frac{1}{2}]  / P[\hat{f}(x+\delta)= l] > 1- \eta
% % % \end{equation}
    
% % %     %\left\{\begin{array}{l}
% % % %f(x+\delta)=\hat{l} \\
% % % %f^{*}(x+\delta)=l
% % % %\end{array}\right.
% % % Let be $ x_{k}^{\prime}=x+\delta_{k}$, and let $x_{k_{0}}^{\prime}$ correspond to the added noise  $\delta_{k_{0}}$ when $x_{k}^{\prime}$ meets the decision boundary:

% % % \begin{equation}
% % % \label{eq:boundary}
% % %     x_{k_{0}}^{\prime}=x+\delta_{k_{0}} / d\left(x_{k_{0}}^{\prime}, B_{f}^{l}\right)=0
% % % \end{equation}

% % % Hence, given Equation \ref{eq:basis}: 
% % % \begin{equation}
% % %     \exists \theta \geqslant 0 \quad / d\left(x, B_{f^{*}}^{l}\right)=d\left(x, B_{f}^{l}\right)+\theta
% % % \end{equation}
% % % Which means, given Equation \ref{eq:boundary}:
% % % \begin{equation}
% % % \label{eq:demo(i)}
% % %     \exists \theta \geqslant 0 / d\left(x_{k_{0}}^{\prime}, B_{f^{\prime}}^{l}\right)=\theta
% % % \end{equation}
% % % Equation \ref{eq:demo(i)} means that while $x_{k}^{\prime}$ is about to be classified by $f$ as $\hat{l}\neq l$, the still is a margin of distortion $\theta$ needed to fool the classifier $f^*$, thus (i).\\

% % % To prove (ii), let be $\hat{x}$ an adverdarial example crafted for $f^*$.  Let be $\beta / f^{*}(\hat{x})= f^{*}(x+\beta)=\hat{l} \neq l$.


% % % \begin{equation}
% % %     d\left(x+\beta, B_{f^{*}}\right)=- \kappa
% % % \end{equation}
% % % Where $\kappa$ is referred to as the confidence margin. 
% % % \begin{equation}
% % %     \exists \alpha \geqslant 0 \quad /  d\left(x+\beta, B_{f^*}^{l}\right)=d\left(x+\beta, B_{f}^{l}\right)+\alpha
% % % \end{equation}

% % % \begin{equation}
% % %     \Rightarrow d\left(x+\beta, B_{f}\right)=-\alpha-k
% % % \end{equation}

% % % \begin{equation}
% % %     \Rightarrow f(x+\beta) \neq L
% % % \end{equation}

% % \begin{figure*}[!htp]
% % \centering
% % \includegraphics[width=2.1\columnwidth]{fexact_fappx-converti.pdf}
% % \caption{A 2D sample space illustration for a) a generated adversarial example for a target classifier and other classifiers under different settings: b) grey-box, c) black-box, and d) white-box.}
% % \label{proxy}
% % \end{figure*}


==> asplos21main-p898-p (Copy)/theory.tex <==

%\begin{appendices}
% \section{Appendix: Theoretical Analysis} \label{sec:theory} %HEREx\nael{Need to come up with a better title for this section}
% %----------------------------------
% We now explore the impact of approximation on the classifier robustness leveraging some formulations from Differential Privacy (DP)~\cite{diff_priv}. %Before proceeding further, note that our purpose in this subsection is not to provide a definitive argument about using approximate computing to defend against adversarial attacks, but rather we view it as an initial step towards drawing an explanation that connects the circuit-level approximation to the model robustness for future work to build upon. 
% %Specifically, while the explainability of deep neural networks behavior is a challenging task, especially under adversarial settings, we attempt to provide an overview on the mechanisms that we think are behind the defensive approximation impact on security. 
% %\ihsen{Attempt starts here}\\
% Our formulation is based on recent similar formulations for certified robustness analysis~\cite{smooth,snP2019_certif}. These prior works studied the impact of randomization on robustness by adding random Gaussian noise to all layers of a CNN.%HEREx\nael{Random is imprecise -- is Gaussian accurate?  If not, what distributions of noise did they consider?} 
% While the noise injected by DA follows a different distribution and is input dependent rather than stochastic, we believe that the theoretical analysis provides insights into the possible mechanisms that improve the robustness of DA.
% %is a theoretical analogy with our work that we develop in the following.   

% In this analysis, we formally model the problem as follows:
% Let $x$ be an input sample and $h$ a conventional classifier. We denote $\hat{h}(x) = h(x) + \triangle(x)$ the defender implementation where $\triangle(x)$ is the data dependent randomness added by the approximate circuit. In this analysis, we use the concept of Differential Privacy (DP) \cite{diff_priv}, \cite{DP}, which is concerned whether the output of a computation over a given database can reveal information about individual records in the database. %In the context of insuring data privacy, these papers suggest injecting a level of randomness 
% To prevent such data leakage, randomness is introduced in the computation, and DP is accordingly defined as follows: 

% \begin{definition} 
%     A randomized algorithm $A$ that takes as input a database $d$ and outputs a value in a space $O$ is said to satisfy ($\varepsilon$, $\delta$)-DP w.r.t. a metric $\rho$ if, for any databases $d$ and $d^{\prime}$ with $\rho(d,d^{\prime}) \leqslant1$, and for any subset of possible outputs $S \subseteq O$, we have:
%     \begin{equation}
%         P(A(d) \in S) \leq e^{\varepsilon} P\left(A\left(d^{\prime}\right) \in S\right)+\delta
%     \end{equation}
% \end{definition}

% Out of this definition, Expected Output Stability Bound, a key property of DP is deduced; the expected value of an ($\varepsilon$, $\delta$)-DP algorithm with bounded output is not sensitive to small changes in the input.
% %\ihsen{next lemma needs more introduction, to match randomization to approximation. A small figure would be perfect. UPDATE: actually we do not need to bring this Lemma here. Go directly to corollary! UPDATE: Nope, the rest of the logic doesn't make sense. Keep it -for now-}


% % \begin{lemma}
% % \label{lemma1}
% % Suppose a randomized function $A$, with bounded output $A(x) \in [0, b], b \in \mathbb{R}^{+}$, satisfies $(\varepsilon, \delta)$-DP. Then the expected output meets the following property: 
% % \begin{center}
% %     $\forall \alpha \in B_{p}(1) . \mathbb{E}(A(x)) \leq e^{\epsilon} \mathbb{E}(A(x+\alpha))+b \delta$
% % \end{center}
% % \end{lemma}

% The intuition behind using the analogy with DP in the context of robustness to adversarial examples is to create an approximate classifier such that, given an input example, the predictions are DP with regards to the features of the input (e.g., the pixels of an image). In this setting, we can derive stability bounds for the expected output of the randomized classifier, i.e., the approximate classifier. The bounds can be interpreted as a certification for robustness to adversarial examples. In our method, the added approximate noise $\triangle(x)$ for a given input $x$ has a similar effect to randomization.


% Formally, to frame the DP into our setting, regard the feature values (e.g., pixels) of an input $x$ as the records in a database.  Let $B_{p}(r):=\left\{\alpha \in \mathbb{R}^{n}:\|\alpha\|_{p} \leq r\right\}$ be the $p$-norm ball of radius $r$. For a given classification model, $h$, and a fixed input, $x \in \mathbb{R}
% ^n$, an attacker is able to craft a successful adversarial example of size $L$ for a given $p$-norm if they find $\alpha \in  B_{p}(L)$ such that $h(x + \alpha) \neq h(x)$. Now, consider an approximate classifier $\hat{h}$ that, on input $x$, outputs scores $\left(y_{1}(x), \ldots, y_{K}(x)\right) \text { (with } y_{k}(x) \in[0,1]$ and $\sum_{k=1}^{K} y_{k}(x)=1)$. 


% Combining Lemma $1$ and Corollary $1$ in \cite{snP2019_certif} directly implies bounds on the expected output on an approximate classifier:
% \begin{theorem}
% Suppose an approximate function $\hat{h}$ satisfies $(\varepsilon, \delta)$-DP w.r.t. a $p$-norm metric, and where $\hat{h}(x)=\left(y_{1}(x), \ldots, y_{K}(x)\right), y_{k}(x) \in[0,1]$:
% \begin{equation}
% \label{eq:dp}
%     \forall k, \forall \alpha \in B_{p}(1) . \hat{h}_{k}(x) \leq e^{\varepsilon} \hat{h}_{k}(x+\alpha) +\delta.%~ \footnote{This corollary and the detailed proofs can be found in \cite{snP2019_certif}} 
% \end{equation}
% \end{theorem}

% Now, consider $\alpha \in B_p(1)$, and let $x^* = x + \alpha$. From Equation \ref{eq:dp}, we have: \textbf{(i)} $\hat{h}_{k}(x) \leqslant e^\varepsilon \hat{h}_{k}(x^*) + \delta$, and
% \textbf{(ii)} $\hat{h}_{i\neq k}(x^*) \leqslant e^\varepsilon \hat{h}_{i\neq k}(x) + \delta$.

% Practically, \textbf{(i)} gives a lower-bound on $\hat{h}_{k}(x^*)$ and \textbf{(ii)} gives an upper-bound on  $\hat{h}_{i\neq k}(x^*)$.

% These elements confirm a theoretically verifiable bounded impact of an adversarial perturbation in the input on the approximate classifier's output. 


% To further investigate the robustness guarantee, suppose that when the base classifier $h$ classifies an input $x$ the most probable class $k$ is returned with probability $p_k$, and the “runner-up” class is returned with probability $p_{i\neq k}< p_k$. Based on \cite{smooth}, our approximate classifier is robust around $x$ within the $\ell_{2} \text { radius } R=\frac{\sigma}{2}\left(\Phi^{-1}\left(p_{k}\right)-\Phi^{-1}\left(p_{i}\right)\right)$, where $\Phi^{-1}$ is the inverse of the standard Gaussian CDF. This result also holds if we replace $p_k$ with a lower bound $\underline{{p}_{k}}$  and we replace $p_i$ with an upper bound $\overline{p_{B}}$. Hence, based on Theorem 1 in \cite{smooth}:

% \begin{theorem}
% \label{theorem:smooth}
% Let  $h: \mathbb{R}^{d} \rightarrow \mathcal{Y}$ be any baseline classifier, and let $\varepsilon \sim \mathcal{N}\left(0, \sigma^{2} I\right)$. Let $\hat{h}$ be the approximate implementation of $h$. Suppose $c_{k} \in \mathcal{Y} \text { and } \underline{p_{k}}, \overline{p_{i}} \in[0,1]$ satisfy:

% \begin{equation}
%     \mathbb{P}\left(h(x+\varepsilon)=c_{k}\right) \geq \underline{p}_{k} \geq \overline{p_{i}} \geq \max _{c \neq c_{k}} \mathbb{P}(h(x+\varepsilon)=c)
% \end{equation}

% Then $\hat{h}(x+ \delta) = c_k$ for all $\|\delta\|_{2}<R$, where 
% \begin{equation}
% \label{eq:theorem_smooth}
%     R=\frac{\sigma}{2}\left(\Phi^{-1}\left(\underline{p_{k}}\right)-\Phi^{-1}(\overline{p_{i}})\right)
% \end{equation}

% \end{theorem}

% Notice that Theorem \ref{theorem:smooth} insures a certified radius $R$ that is large when: (1) the noise level $\sigma$ is high, (2) the probability of the top class $c_k$ is high, and (3) the probability of each other class $c_{i \neq k}$ is low.

% Conditions (2) and (3) of high radius basically mean a higher confidence in the sense of Equation \ref{eq:confidence}. This is coherent with the results obtained in terms of robustness, given Figure \ref{conf_dis}.

% The randomization technique proposed in \cite{snP2019_certif} and \cite{smooth} uses a totally random noise that is uncorrelated to the input. This led them to use heavy Monte Carlo simulations to estimate the randomized classifier's output, which induces a considerable time overhead limiting the applicability of these techniques, especially in time critical applications. In our approach, the noise is injected at circuit-level through the approximate design and is not artificially generated from an outside source. Moreover, the correlation to the input that highlights useful features in the convolution output gives higher confidence and thereby ensures a higher robustness radius in the sense of Theorem \ref{theorem:smooth}.

\section{Appendix: Design Space Exploration} \label{sec:DSE}
\textbf{Accuracy.} HEAP \cite{Heap} is the result of a design space exploration among combinations of different approximate full adders leading to minimal accuracy loss. The selection process of optimal circuit design was performed after an exhaustive accuracy evaluation of all possible configurations.% The exploration was performed as described in \textbf{Algorithm 1}
The metrics used to evaluate the accuracy of different combinations are the mean relative error distance (MRED) \cite{metrics} $ {\textstyle MRED= \frac{1}{n} \sum_{i=1}^{n} \frac{ \mid{\hat Y -Y}\mid}{Y} }$, and the normalized mean error distance (NMED): ${\textstyle NMED= \frac{1}{n} \sum_{i=1}^{n} \frac{ \mid{\hat Y -Y}\mid}{P_{max}} }$. Where $Y$ is the exact result, $ \hat Y $ is the approximate result, and $P_{max}$ is the maximum product.

%\begin{algorithm}
%\caption{DSE Algorithm}
%\begin{algorithmic}[1]
%\State \textbf{Input:} POPSIZE //size of the population;\\
%C //Error constraint;
%\State \textbf{Output:} final combination
%%\textit{//Initialize population:}
%\State i = 0;
%\While {i < POPSIZE}
%\State Generate random combination;
%\State Calculate the NMED;
%\If {NMED < C}
%\State Add the new combination to the population;
%\State i++;
%\EndIf
%\EndWhile
%%\State \textit{//Minimize fitness function:}
%\Repeat
%\State Calculate the fitness of each combination;
%\State Sort population according to fitness;
%%\State \textit{//Generate new population:}
%\State Select the \textit{best} individuals to reproduce;
%\State Generate new offspring using crossover and mutation
%\State Calculate the NMED of the new offspring;
%\If {NMED < C}
%\State Add the offspring to the new population;
%\EndIf
%\Until no improvement
%\end{algorithmic}
%\end{algorithm}
\begin{table}[!htp]
\centering
  \caption{Accuracy results of the LeNet-5 CNN and different multipliers.}
  \label{tab3}
  \begin{tabular}{cccc}
    \toprule
    \textbf{Multiplier }& \textbf{CNN Accuracy}	& \textbf{MRED} & \textbf{NMED}	 \\
    \midrule
        Exact multiplier        & 97.93\%  & 0    & 0\\
        HEAP \cite{Heap}        & 97.86\%  & 0.12 & 0.03\\
        Ax-FPM	    & 97.67\%  & 0.33 & 0.08\\ 
  \bottomrule
\end{tabular}
\end{table}

Table \ref{tab3} includes the accuracy results of the exact multiplier and the two approximate multipliers.
Ax-FPM is substantially less accurate than HEAP.  However, when we evaluate CNN accuracy (using the recognition rate), we notice a negligible accuracy loss for both approximate multipliers, confirming the inherent error-resiliency of CNNs.

\begin{figure}[!htp]
\centering
\includegraphics[width=0.9\columnwidth,height=3.5cm]{error_dis__8_.pdf}
\caption{Noise introduced by the approximate multiplier while the operands $\in [0,1]$ (a). for Ax-FPM, (b). for HEAP \cite{Heap}. 
}
\label{appx_mult_heap}
\end{figure}
Measuring the error introduced by the Ax-FPM and the HEAP for small inputs ranging between $0$ and $1$, see Figure \ref{appx_mult_heap}, we notice that, in addition to the smaller magnitude of error when using the HEAP, a different pattern was found: less data dependency and for only $34\%$ of the cases, the HEAP results were higher than the exact multiplier results. 

In order to further investigate the impact of different approximate multipliers on the convolution layer output, we produce different heat maps. As shown in Figure \ref{heatmaps}, we can see that the Ax-FPM is further highlighting the important features by increasing their scores whereas the HEAP is lowering their scores.

\begin{figure}[!htp]
\centering
\includegraphics[width=0.9\columnwidth]{Heatmaps.pdf}
\caption{ Heat maps of final convolution layer output when using Exact multiplier, Ax-FPM, and HEAP \cite{Heap}. }
\label{heatmaps}
\end{figure}

\noindent\textbf{Energy consumption and Delay.}
We also compare the gain in terms of energy and delay achieved by the two approximate mantissa multipliers. Multipliers are implemented using $45~ n m$ technology via the Predictive Technology Model (PTM) using the Keysight Advanced Design System (ADS) simulation platform~\cite{PTM}.   

\begin{table}[!htp]
\centering
  \caption{Energy and delay of different $24\times24$ approximate multipliers normalized to a conventional $24\times24$ multiplier.}
  \label{tab}
  \begin{tabular}{ccc}
    \toprule
    \textbf{Multiplier }& \textbf{Average energy}	& \textbf{Average delay}  	 \\
    \midrule
        Exact multiplier        & 1 & 1    \\
        HEAP                    & 0.49  & 0.46\\
        Ax-FPM	                 & 0.395 & 0.235\\ 
  \bottomrule
\end{tabular}
\end{table}

As shown in Table \ref{tab}, the mantissa multiplier in Ax-FPM achieves a considerable gain in performance and energy saving compared to the HEAP. A significant reduction in the delay was also achieved.  

\noindent\textbf{Robustness.}
We tried to assess different models transferability, the adversarial examples were generated to fool the exact model. In table \ref{grey-boxresult_with_heap}, we present the percentage of adversarial examples that successfully deceived the approximate models. While the use of the HEAP increased the robustness of the model, the Ax-FPM achieved better results.

\begin{table}[!htp]
\small
\centering
  \caption{Attacks transferability success rates for MNIST.}
  \label{grey-boxresult_with_heap}
  \begin{tabular}{cccc}
    \toprule
    \textbf{Attack} & \textbf{Exact-based}  & \textbf{HEAP-based} & \textbf{Ax-FPM-based}\\
    \midrule
        FGSM          &   100\%  & 16\% & 12\%    \\
        PGD           &   100\%  & 30\% & 28\%    \\
        JSMA          &   100\%  & 42\% & 9\%   \\
        C\&W          &   100\%  & 6\% & 1\%    \\
        DF	          &   100\%  & 18\%  & 17\%   \\ 
        LSA	          &   100\%  & 41\% & 18\%   \\ 
        BA	          &   100\%  & 22\% & 17\%   \\ 
        HSJ	          &   100\%  & 4\% & 2\%    \\         
  \bottomrule
\end{tabular}
\end{table}

All these results confirm that Ax-FPM is a better choice in terms of robustness and resource and power efficiency.

\section{Appendix: Defensive Quantization: Models Architecture}
\label{mod_archi}
We present models architectures in Table \ref{architecture}: For the fully quantized model, ConvolutionQuant, DenseQuant and reluQuant designate respectively a convolution layer with quantized weights, a dense layer with quantized weights and the relu activation function with its output quantized. For the weight quantized model architecture, the ConvolutionQuant and DenseQuant designate respectively a convolution layer with quantized weights and a dense layer with quantized weights.

\begin{table}[!htp]
\small
\centering
  \caption{Fully quantized and Weight quantized models architecture.}
  \label{architecture}
  \begin{tabular}{cc}
    \toprule
    \textbf{Fully Quantized} & \textbf{Weight Quantized}  \\
    \midrule
        ConvolutionQuant     &  ConvolutionQuant    \\
        BatchNorm            &  BatchNorm   \\
        reluQuant            &  relu    \\
        ConvolutionreluQuant &  ConvolutionreluQuant    \\
        MaxPooling           &  MaxPooling    \\
        BatchNorm            &  BatchNorm    \\
        reluQuant            &  relu  \\
        ConvolutionQuant     &  ConvolutionQuant    \\
        BatchNorm            &  BatchNorm     \\
        reluQuant            &  relu \\
        ConvolutionQuant     &  ConvolutionQuant    \\
        MaxPooling           &  MaxPooling    \\
        BatchNorm            &  BatchNorm    \\
        reluQuant            &  relu \\
        ConvolutionQuant     &  ConvolutionQuant    \\
        BatchNorm            &  BatchNorm    \\
        reluQuant            &  relu\\
        ConvolutionQuant     &  ConvolutionQuant    \\
        MaxPooling           &  MaxPooling    \\ 
        BatchNorm            &  BatchNorm    \\
        reluQuant            &  relu    \\
        DenseQuant           &  DenseQuant    \\
        BatchNorm            &  BatchNorm    \\
        reluQuant       	 &  relu   \\ 
        DenseQuant           &  DenseQuant    \\
        BatchNorm            &  BatchNorm    \\
        reluQuant	         &  relu    \\ 
        Dense                &  Dense    \\
        softmax	             &  softmax    \\ 
               
  \bottomrule
\end{tabular}
\end{table}

%\end{appendices}
